Trimming the Fat: Efficient Compression of 3D Gaussian Splats through Pruning

In recent times, the utilization of 3D models has gained traction, owing to the capacity for end-to-end training initially offered by Neural Radiance Fields and more recently by 3D Gaussian Splatting (3DGS) models. The latter holds a significant advantage by inherently easing rapid convergence during training and offering extensive editability. However, despite rapid advancements, the literature still lives in its infancy regarding the scalability of these models. In this study, we take some initial steps in addressing this gap, showing an approach that enables both the memory and computational scalability of such models. Specifically, we propose "Trimming the fat", a post-hoc gradient-informed iterative pruning technique to eliminate redundant information encoded in the model. Our experimental findings on widely acknowledged benchmarks attest to the effectiveness of our approach, revealing that up to 75% of the Gaussians can be removed while maintaining or even improving upon baseline performance. Our approach achieves around 50$\times$ compression while preserving performance similar to the baseline model, and is able to speed-up computation up to 600 FPS.

==> bmvc_paper.tex <==
% \documentclass{bmvc2k}

% \usepackage{graphicx}
% \usepackage{cleveref}
% \usepackage{multirow}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{booktabs}
% \usepackage{wrapfig}
% \usepackage{enumitem}
% \newcommand{\salman}[1]{\textcolor{blue}{#1}}
% \newcommand{\enzo}[1]{\textcolor{red}{#1}}

% \hbadness=10000 % Suppress "Underfull \hbox" warnings

% %% Enter your paper number here for the review copy
% \bmvcreviewcopy{358}

% \title{Trimming the Fat: Efficient Compression of 3D Gaussian Splats through Pruning}

% % Enter the paper's authors in order
% % \addauthor{Name}{email/homepage}{INSTITUTION_CODE}
% \addauthor{Susan Student}{http://www.vision.inst.ac.uk/~ss}{1}
% \addauthor{Petra Prof}{http://www.vision.inst.ac.uk/~pp}{1}
% \addauthor{Colin Collaborator}{colin@collaborators.com}{2}

% % Enter the institutions
% % \addinstitution{Name\\Address}
% \addinstitution{
%  The Vision Institute\\
%  University of Borsetshire\\
%  Wimbleham, UK
% }
% \addinstitution{
%  Collaborators, Inc.\\
%  123 Park Avenue,\\
%  New York, USA
% }

% \runninghead{Student, Prof, Collaborator}{BMVC Author Guidelines}

% % Any macro definitions you would like to include
% % These are not defined in the style file, because they don't begin
% % with \bmva, so they might conflict with the user's own macros.
% % The \bmvaOneDot macro adds a full stop unless there is one in the
% % text already.
% \def\eg{\emph{e.g}\bmvaOneDot}
% \def\Eg{\emph{E.g}\bmvaOneDot}
% \def\etal{\emph{et al}\bmvaOneDot}

% %-------------------------------------------------------------------------
% % Document starts here
% \begin{document}

% \maketitle




% \begin{abstract}
% %In recent times, the utilization of 3D models has gained traction, owing to the capacity for end-to-end training initially offered by Neural Radiance Fields and more recently by 3D Gaussian Splatting (3DGS) models. The latter holds a significant advantage by inherently facilitating rapid convergence during training and offering extensive editability. However, despite advancements, the literature still lacks exploration into the scalability of these models. In this study, we take the initial steps in addressing this gap showing an approach that enables both the memory and computational scalability of such models. Specifically, we propose an iterative pruning technique to eliminate redundant information encoded in the model. We show that a simple magnitude-based approach achieves subpar results when compared to a gradient-informed one, despite traditional pruning literature showing that not being the typical case. Our experimental findings on widely acknowledged benchmarks attest to the effectiveness of our approach, revealing that up to 75\% of the Gaussians can be removed while maintaining or even improving upon baseline performance. Given that the pruned Gaussians are entirely eliminated, this directly influences the scalability of the Gaussians, thus indicating the potential for widespread deployment, even on devices with limited resources. By integrating our pruning method with an end-to-end compression approach for 3D Gaussian Splatting (3DGS), we attain state-of-the-art compression performance. Our combined approach achieves compression rates of around 50$\times$, while preserving performance similar to the baseline model. We commit to release the code open-source upon acceptance of the article.
% In recent times, the utilization of 3D models has gained traction, owing to the capacity for end-to-end training initially offered by Neural Radiance Fields and more recently by 3D Gaussian Splatting (3DGS) models. The latter holds a significant advantage by inherently easing rapid convergence during training and offering extensive editability. However, despite rapid advancements, the literature still lives in its infancy regarding the scalability of these models. In this study, we take some initial steps in addressing this gap, showing an approach that enables both the memory and computational scalability of such models. Specifically, we propose ``Trimming the fat'', a post-hoc gradient-informed iterative pruning technique to eliminate redundant information encoded in the model. %We show that a simple magnitude-based approach achieves subpar results when compared to a gradient-informed one, despite traditional pruning literature showing that not being the typical case. 
% Our experimental findings on widely acknowledged benchmarks attest to the effectiveness of our approach, revealing that up to 75\% of the Gaussians can be removed while maintaining or even improving upon baseline performance. %By integrating our pruning method with an end-to-end compression approach for 3D Gaussian Splatting (3DGS), we attain state-of-the-art compression performance. 
% Our approach achieves around 50$\times$ compression while preserving performance similar to the baseline model, and is able to speed-up computation up to 600~FPS. We commit to release the code open-source upon acceptance of the article.
% \end{abstract}

% %-------------------------------------------------------------------------
% \section{Introduction}
% \label{sec:intro}
% \begin{wrapfigure}{r}{0.7\textwidth}
%     \vspace{-10pt}
%     \centering
%     \includegraphics[width=0.99\linewidth]{Figures/Teaser_try_again1.pdf}
%     \caption{%Comparison of 3DGS-30k with Niedermayr's Compression, our pruning method, and their combination yields compelling results. Our pruning compresses scenes by up to 4.5$\times$ without sacrificing visual quality. It seamlessly integrates with any compression method. Combined with Niedermayr's approach, we achieve up to 60$\times$ compression with similar visual quality.
%     Vanilla 3DGS-30k VS our novel pruning approach applied with an end-to-end compression technique~\cite{niedermayr2023compressed}.% Our pruning method achieves scene compression of up to 7.5$\times$ without compromising visual fidelity, integrating smoothly with diverse compression methods. When paired with the Niedermayr et al. method~\cite{niedermayr2023compressed}, we achieve compression rates of up to 60$\times$ while preserving comparable visual quality.}
%     }
%     \label{fig:teaser}
%     \vspace{-0.4cm}
% \end{wrapfigure}
% In the last few years, significant advancements have been made in radiance field methodologies for reconstructing 3D scenes using images captured from various viewpoints. The emergence of Neural Radiance Fields (NeRF) techniques has notably influenced the realm of 3D scene modeling and reconstruction~\cite{mildenhall2021nerf,huang2022stylizednerf}. The efficient generation of photo-realistic novel views from a given set of training images has become a focal point in computer vision research, with diverse applications~\cite{deng2023compressing}. NeRF's capability to distill the essence of a 3D object from its 2D representations, while maintaining compactness, underscores its impact and popularity in the literature~\cite{yu2021pixelnerf,kaya2022neural}.

% Despite its success, the traditional NeRF~\cite{mildenhall2021nerf} suffers from slow training and rendering speeds. To address this challenge, various approaches have been proposed, although they often entail compromises in rendered image quality~\cite{deng2023compressing}. Recent studies have turned to explicit scene representations, such as voxel-based~\cite{sun2022direct} or point-based~\cite{xu2022point} structures to enhance rendering efficiency. For instance, leveraging 3D voxel grids on GPUs alongside multi-resolution hash encoding of inputs led to consistent reductions in required operations and enabled real-time performance~\cite{muller2022instant}. Similarly, the most efficient radiance field solutions to date rely on continuous representations achieved through interpolating values stored in voxel~\cite{fridovich2022plenoxels}, hash grids~\cite{muller2022instant}, or points~\cite{xu2022point}. While the continuous nature of these methods aids optimization, the stochastic sampling necessary for rendering can incur computational overhead and introduce noise~\cite{kerbl20233d}.

% % \begin{wrapfigure}{r}{0.5\textwidth}
% %     \centering
% %     \includegraphics[width=0.99\linewidth]{Figures/teaser.pdf}
% %     \caption{Qualitative comparison of our proposed method and original 3DGS-30k. With our proposed method we can achieve compression rates of about $7.5\times$ with indiscernible loss in visual quality simply with proper pruning.}
% %     \label{fig:teaser}
% %     \vspace{-0.4cm}
% % \end{wrapfigure}

% A recent advancement in the field is the introduction of differentiable 3D Gaussian splatting (3DGS), which enables the generation of a sparse adaptive scene representation~\cite{kerbl20233d}. This representation can be rendered rapidly on the GPU, offering big speed improvements. 3DGS combines the best features of existing methods: leveraging a 3D Gaussian representation for scene optimization provides state-of-the-art visual quality and competitive training times while the tile-based splatting solution ensures real-time rendering at high quality for 1080p resolution across various datasets. Unlike NeRF methods, 3DGS simplifies training and rendering by projecting 3D Gaussians to the 2D image space and combines them with opacity using \emph{rasterization}, enabling real-time rendering on a single GPU. Furthermore, the explicit storage of scene structure in the parameter space allows for direct editing of the 3D scene. However, some challenges emerge when employing differentiable 3DGS, particularly in optimizing scenes with millions of Gaussians, which may require substantial storage and memory. While specialized pipelines demonstrate real-time performance on high-end GPUs, seamless integration into VR/AR environments or games remains a challenge, particularly when working alongside hardware rasterization of polygon models.

% In this paper, we aim to compress Gaussian splatting representations while preserving their rendering speed and quality, facilitating their application across diverse domains such as IoT devices with limited storage or memory. Our primary insight is that the learned 3DGS models exhibit over-fitting to the underlying scene, allowing for the removal or pruning of many Gaussians without sacrificing performance, particularly due to markedly lower opacity values. We start the training process with a pre-trained optimized Gaussian scene, iteratively pruning it based on opacity levels and gradient values, followed by fine-tuning to achieve superior performance-compression trade-off compared to the baseline optimized scene as showcased from Fig.~\ref{fig:teaser}. Our main contributions are the following.

% %We start the training process with a pre-trained optimized Gaussian scene, iteratively pruning it based on opacity levels and gradient values, followed by fine-tuning to achieve superior performance compared to the baseline optimized scene. Our main contributions are as follows:

% \begin{itemize}[noitemsep, nolistsep]
%     \item We build on top of the optimized 3DGS as a 3D prior for pruning, enabling the removal of redundant Gaussians while fine-tuning the remaining ones to accurately capture the scene features (Sec.~\ref{sec: pruning}). 
    
%     \item We observe that vanilla pruning is sub-optimal when compared to a gradient-informed approach and that pruning without such a prior fails. Besides, we showcase the compatibility with other compression pipelines, like~\cite{niedermayr2023compressed} (Sec.~\ref{sec:abl}).

%     \item With our proposed method, we achieve state-of-the-art performance even after pruning 50\% of the Gaussian splats, significantly enhancing the scalability of 3DGS (Sec.~\ref{sec:res}). Our compression pipeline achieves an enhanced balance between scene fidelity and compression, surpassing the baseline (Fig.~\ref{fig: Pruning-Comparison-1}). %To the best of our knowledge, our iterative pruning approach stands as the state-of-the-art: when integrated with the existing end-to-end compression approach~\cite{niedermayr2023compressed}, our method achieves a compression ratio of approximately 50$\times$, all while preserving performance metrics akin to those of the baseline (Sec.~\ref{sec:res}).
% \end{itemize}

% %Since the main focus of this work is on showing and discussing the contribution of pruning, although extra compression steps are possible (including vector quantization, entropy coding, Morton ordering etc.) we did not include or compare with them, as it stands out the scope of this work which is a study on the effect of proper pruning to compress 3DGS models.



% \section{Related Work}
% \label{sec:Related Work}
% In this section we first provide an overview of the most recent methods for novel view synthesis (Sec.~\ref{sec:nws}), then we discuss approaches for their compression (Sec.~\ref{sec:3dgs-compress}).

% \subsection{Novel View Synthesis}
% \label{sec:nws}
% Recent advancements in novel view synthesis have seen significant progress, with early techniques using CNNs to estimate blending weights or texture-space solutions~\cite{flynn2016deepstereo, hedman2018deep,riegler2020free,thies2019deferred}, albeit facing challenges with MVS-based geometry and temporal flickering. Volumetric representations, starting with Soft3D~\cite{penner2017soft} and employing deep learning with volumetric ray-marching~\cite{henzler2019escaping,sitzmann2019deepvoxels}, provided further advancements. Neural Radiance Fields (NeRFs)~\cite{mildenhall2021nerf} aimed to enhance synthesized views' quality but faced slow processing due to a large Multi-Layer Perceptron (MLP) backbone and dense sampling. Subsequent methods like Mip-NeRF360~\cite{barron2022mip} focused on balancing quality and speed, while recent advances prioritize faster training and rendering through spatial data structures, encodings, and MLP adjustments~\cite{chen2023mobilenerf,fridovich2022plenoxels,garbin2021fastnerf}. Notable methods such as InstantNGP~\cite{muller2022instant} leverage hash grids and occupancy grids for accelerated computation, while Plenoxels~\cite{fridovich2022plenoxels} rely on Spherical Harmonics for directional effects without neural networks. Despite these strides, challenges persist in NeRF methods regarding efficient coding for empty space, image quality, and rendering speed.

% In contrast, 3DGS achieves superior quality and faster rendering without implicit learning. However, its increased storage compared to NeRF methods poses limitations. Our approach aims to maintain the quality and speed of 3DGS while reducing model storage by applying pruning to Gaussian parameters.
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{Figures/3DGS-overview.pdf}
%     \caption{Overview of our pruning pipeline. From a pre-trained 3DGS-30k scene, we first iteratively prune it for a fixed number of iterations with subsequent fine-tuning. Then, we conduct further fine-tuning for 20,000 iterations to obtain our final optimized scene.}
%     \label{fig:overview}
% \end{figure*}
% %\subsection{NeRFs Compression}
% %\label{sec:compress}
% % Various methods have emerged to address the computational costs associated with NeRF's dense sampling of color values and opacity. These methods adopt different data structures such as trees~\cite{wang2022fourier, yu2021plenoctrees}, point clouds~\cite{peng2021shape,xu2022point}, and grids~\cite{chen2022tensorf, fridovich2022plenoxels, muller2022instant,sun2022direct} to efficiently represent 3D scenes and objects. Grid structures, for instance, enable training iterations to be completed in a matter of minutes, but they may require substantial memory due to their dense nature. To mitigate this, several approaches have focused on reducing the size of volumetric grids~\cite{chen2022tensorf,huang2022pref,takikawa2022variable}. Instant-NGP~\cite{muller2022instant} utilizes hash-based multi-resolution grids, while VQAD~\cite{takikawa2022variable} replaces the hash function with codebooks and vector quantization.  
% %  VQRF~\cite{li2023compressing} compresses volumetric grid-based radiance fields by adopting vector quantization. Additionally, frequency domain transformation~\cite{rho2023masked,zhao2023tinynerf}, and voxel pruning~\cite{deng2023compressing} have also been proposed to reduce the memory consumption of grid-based NeRFs. Despite these efforts, grid-based NeRF variants still have larger sizes compared to MLP-based methods.

% % Although dense voxel-based representations significantly increase rendering speed, they require significantly more memory than implicit volumetric representations. Hierarchical structure representations using octrees offer a sparse encoding of the 3D scene but still exhibit high memory occupancy. Recent work has addressed training models with neural sparse voxel fields~\cite{liu2020neural}, progressively reducing voxel granularity and skipping rendering for empty voxels. However, these approaches primarily focus on performance enhancement and artifact reduction rather than compression.

% %%%%% Methodology section starts here

% % \begin{figure*}[t]
% % \includegraphics[width=\linewidth]{Figures/playroom-pruning-comp.pdf}
% %     \centering
% %     \caption{Qualitative comparison of the playroom scene at various pruning levels, defined by $\gamma$ using gradient-aware iterative pruning. Our proposed method demonstrates substantially higher compression rates compared to both baselines while maintaining similar visual quality.}
% %     \label{fig: Pruning-Comparison-2}
% %     %\vspace{-0.4cm}
% % \end{figure*}


% % \begin{figure*}[t]
% % \includegraphics[width=\linewidth]{Figures/train-pruning-comp.pdf}
% %     \centering
% %     \caption{Qualitative comparison of the train scene at various pruning levels, defined by $\gamma$ using gradient-aware iterative pruning. Our proposed method demonstrates substantially higher compression rates compared to both baselines while maintaining similar visual quality.}
% %     \label{fig: Pruning-Comparison-3}
% %     %\vspace{-0.4cm}
% % \end{figure*}
% \subsection{3DGS Compression}
% \label{sec:3dgs-compress}
% When compared to NeRFs, 3DGS models lack structure, which presents challenges for compression~\cite{chen2024hac,fei20243d}. Consequently, many studies in 3DGS compression introduce structural parameters by replacing vanilla 3DGS parameters to enhance compression~\cite{lu2023scaffold, chen2024hac}. Scaffold-GS~\cite{lu2023scaffold}, for instance, utilizes anchor points to distribute local 3D Gaussians and predicts their attributes dynamically based on the viewing direction and distance within the view frustum. On the other hand, the Hash-grid Assisted Context (HAC)~\cite{chen2024hac} framework jointly learns a structured compact hash grid and uses it for context modeling of anchor attributes. %Specifically, with Scaffold-GS~\cite{lu2023scaffold} as their base model, for each anchor, they query the hash grid by the anchor location to obtain an interpolated hash feature, which is then used to predict the value distributions of anchor attributes, facilitating entropy coding.

% Niedermayr~\etal~\cite{niedermayr2023compressed} proposed a compression framework that maintains vanilla 3DGS parameters while compressing directional colors and Gaussian parameters. This framework incorporates sensitivity-aware vector clustering and quantization-aware training and achieves compression rates of up to 30$\times$ with a marginal decline in performance compared to the baseline 3DGS. Another method, Compact3D~\cite{lee2023compact}, introduces a learnable mask strategy to prune the Gaussians and a compact representation of view-dependent colors by employing a grid-based neural field rather than relying on spherical harmonics. It also learns codebooks to compactly represent the geometric attributes of Gaussian by vector quantization.

% Our proposed pruning method can effectively improve/replace the masking strategies for unimportant Gaussians in the existing works (see Sec.~\ref{sec:res}). However, for the scope of this paper and considering the broad applicability of vanilla 3DGS, we focus solely on the vanilla 3DGS variant.

% % \salman{When compared to NeRFs, 3D Gaussian Splatting (3DGS) models lack structure, posing challenges for compression. Consequently, the majority of studies in 3DGS compression introduce structural parameters by replacing vanilla 3DGS parameters to enhance compression~\cite{lu2023scaffold, fan2023lightgaussian, lee2023compact, chen2024hac, morgenstern2023compact}. Niedermayr et al.~\cite{niedermayr2023compressed} proposed a compression framework that maintains vanilla 3DGS parameters while compressing directional colors and Gaussian parameters. This framework incorporates sensitivity-aware vector clustering and quantization-aware training and achieves compression rates of up to 30$\times$ with a marginal decline in performance compared to the baseline 3DGS. Our pruning approach can seamlessly integrate with these end-to-end compression methods. However, for the scope of this paper and considering the broad applicability of vanilla 3DGS, we focus solely on the vanilla 3DGS variant.}

% \section{Methodology}
% %Despite the impressive performance and enhanced editability of 3DGS models, their substantial storage memory requirements often pose challenges, necessitating significant memory resources. 
% In this section, we first provide an overview of the 3DGS technique for learning and rendering 3D scenes, as introduced by Kerbl~\etal~\cite{kerbl20233d} (Sec.~\ref{sec: 3DGS}). Then, we delve into an explanation of our pruning approach (Sec.~\ref{sec: pruning}). Our methodology, depicted in Fig.~\ref{fig:overview}, introduces an effective approach to compress these models using gradient-informed pruning.
% %In this section, we first provide an overview of the 3D Gaussian Splatting (3DGS) technique for learning and rendering 3D scenes, as introduced by Kerbl et al.~\cite{kerbl20233d} (Sec~\ref{sec: 3DGS}). Despite their remarkable performance and enhanced editability, 3DGS models are hindered by their considerable storage memory requirements, often necessitating substantial memory resources. Our methodology, outlined in Figure \ref{fig:overview}, introduces a simple yet effective approach to compress these models using pruning technique (Sec~\ref{sec: pruning}).
% %First, we present an overview of the 3D Gaussian Splatting (3DGS)~\cite{kerbl20233d} technique for learning and rendering 3D scenes, followed by an explanation of our pruning approach.


% \subsection{Differentiable Gaussian Splatting}
% \label{sec: 3DGS}
% 3DGS~\cite{kerbl20233d} represents a scene through a set of 3D Gaussians. By leveraging differentiable Gaussian splatting, which extends EWA volume splatting~\cite{zwicker2001ewa}, it facilitates the efficient projection of 3D Gaussian kernels onto the 2D image plane. Additionally, differentiable rendering optimizes the quantity and attributes of the Gaussian kernels employed to characterize the scene. Each 3D Gaussian is characterized by its position and covariance matrices within the 3D space, modeled as
% \vspace{-10pt}
% \begin{equation}
% G(x)=\exp\left[-\frac{1}{2}(x-\mu)^T \Sigma^{-1}(x-\mu)\right],
% \vspace{-5pt}
% \end{equation}

% where \(x\) denotes the position vector, \(\mu\) represents the position, and \(\Sigma\) is the 3D covariance matrix of the Gaussian distribution. Given the requirement for the covariance matrix to be positive definite, it can be parameterized using a rotation matrix \(R\) and a scaling matrix \(S\). To facilitate independent optimization of \(R\) and \(S\), Kerbl~\etal~\cite{kerbl20233d} introduce a representation of rotation via a quaternion \(q\) and scaling through a vector \(s\), both of which can be converted into their corresponding matrices. Additionally, each Gaussian distribution possesses its opacity (\(\alpha \in [0, 1]\)) and a set of spherical harmonics (SH) coefficients essential for reconstructing a view-dependent color. The 2D projection of a 3D Gaussian remains a Gaussian with covariance
% \begin{equation}
%     \Sigma' = JW\Sigma W^TJ^T,
%     \vspace{-5pt}
% \end{equation}
% \noindent
% where \(W\) is the view transformation matrix, and \(J\) is the Jacobian of the affine approximation of the projective transformation. This setup facilitates the evaluation of the 2D color and opacity footprint of each projected Gaussian. The color \(C\) of a pixel is subsequently determined by blending all the \(N\) 2D Gaussians contributing to that pixel:%, %with blending performed in sorted order thanks to the GPU efficient rasterization process, 
% %defined as
% \vspace{-10pt}
% \begin{equation}
%     C = \sum_{i \in N} c_i \alpha_i + \prod_{j=1}^{i-1} (1 - \alpha_j),
% \end{equation}

% \noindent
% where \(c_i\) and \(\alpha_i\) represent the view-dependent color and opacity of a Gaussian, respectively, which are adjusted based on the exponential decay from the center point of the projected Gaussian. The parameters such as position \(x\), rotation \(q\), scaling \(s\), opacity \(\alpha\), and spherical harmonics (SH) coefficients of each 3D Gaussian are optimized to ensure alignment between the rendered 2D Gaussians and the training images.

% During the training phase, the 3D Gaussian splats are rendered efficiently in a differentiable manner to produce a 2D image. This rendering process involves $\alpha$-blending of anisotropic splats, sorting them, and utilizing a tile-based rasterizer. At each training iteration, the 3DGS framework renders the training viewpoints and then minimizes the loss between the ground truth and rendered images in the pixel space, where the loss is given by 
% \vspace{-5pt}
% \begin{equation}
% \mathcal{L}=(1-\lambda) \mathcal{L}_1+\lambda \mathcal{L}_{\text {D-SSIM }},
% \vspace{-5pt}
% \end{equation}

% \noindent
% %$\lambda$= 0.2 is employed consistently across all our experiments. For more details please refer to the 3DGS paper \cite{kerbl20233d}.
% where $\mathcal{L}_1$ is the $\ell_1$ norm of the rendered output and $\mathcal{L}_{\text {D-SSIM }}$ is its structural dissimilarity. The optimization in 3DGS begins with a point cloud generated through a conventional SfM method~\cite{ullman1979interpretation}, and then proceeds iteratively, pruning Gaussians with small opacity parameters and introducing new ones when significant gradients are detected. As demonstrated in the 3DGS paper, this approach enables rapid training and facilitates real-time rendering, all while achieving comparable or superior 3D model quality compared to state-of-the-art NeRF methods.

% %\subsection{Compressing Gaussian Splats}
% %While 3DGS models exhibit impressive performance and offer enhanced editability, they suffer from significant storage memory requirements, often demanding substantial memory resources. In our methodology as shown in \cref{fig:overview}, we introduce a straightforward yet powerful approach to compress these models using pruning technique.


% % \begin{table*}[t]

% %     \centering
% %     \scalebox{0.99}{
% %     \begin{tabular}{cccc|cccc}
% %     \toprule
% %     \multicolumn{4}{c}{One Shot Pruning} & \multicolumn{4}{c}{Iterative Pruning} \\
% %     SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem  &SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem \\
% %     \midrule
% %     0.848 & 23.920 & 0.171 & 326.75 & 0.849 & 23.981 & 0.169 & 338.5 \\
% %     0.848 & 23.901 & 0.172 & 261.5 & 0.849 & 23.939 & 0.171 & 261 \\
% %     0.844 & 23.813 & 0.180 & 196.25 & 0.846 & 23.961 & 0.178 & 200 \\
% %     0.839 & 23.698 & 0.191 & 152.75 & 0.839 & 23.799 & 0.192 & 152 \\
% %     0.819 & 23.376 & 0.228 & 87.5 & 0.818 & 23.404 & 0.232 & 86 \\
% %     0.793 & 22.927 & 0.272 & 44 & 0.794 & 23.069 & 0.574 & 47 \\
% %     0.756 & 22.234 & 0.322 & 22 & 0.767 & 22.655 & 0.310 & 25 \\
% %     \bottomrule
% %     \end{tabular}    
% %     }
% %     \caption{Performance comparison between one-shot pruning and iterative pruning on Tanks\&Temples dataset. Memory size is in MBs.}
% %     \label{tab: one-shot-pruning_comp}
% % \end{table*}

% % \begin{table}[t]
% %     \centering
% %     \scalebox{0.75}{
% %     \begin{tabular}{cccc|cccc}
% %     \toprule
% %     \multicolumn{4}{c}{One Shot Pruning} & \multicolumn{4}{c}{Iterative Pruning} \\
% %     SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem  &SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem \\
% %     \midrule
% %     0.848 & 23.920 & 0.171 & 326.75 & 0.849 & 23.981 & 0.169 & 338.50 \\
% %     0.848 & 23.901 & 0.172 & 261.50 & 0.849 & 23.939 & 0.171 & 261.00 \\
% %     0.844 & 23.813 & 0.180 & 196.25 & 0.846 & 23.961 & 0.178 & 200.00 \\
% %     0.839 & 23.698 & 0.191 & 152.75 & 0.839 & 23.799 & 0.192 & 152.00 \\
% %     0.819 & 23.376 & 0.228 & 87.50 & 0.818 & 23.404 & 0.232 & 86.00 \\
% %     0.793 & 22.927 & 0.272 & 44.00 & 0.794 & 23.069 & 0.574 & 47.00 \\
% %     0.756 & 22.234 & 0.322 & 22.00 & 0.767 & 22.655 & 0.310 & 25.00 \\
% %     \bottomrule
% %     \end{tabular}    
% %     }
% %     \caption{Performance comparison between one-shot pruning and iterative pruning on Tanks\&Temples dataset. Memory size is in MBs.}
% %     \label{tab:one-shot-pruning_comp}
% % \end{table}

% % \begin{table*}


% %     \centering
% %     \scalebox{0.99}{
% %     \begin{tabular}{cccc|cccc}
% %     \toprule
% %     \multicolumn{4}{c}{Opacity Aware Pruning} & \multicolumn{4}{c}{Gradient Aware Opacity Pruning} \\
% %     SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem  &SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem \\
% %     \midrule
% %         0.849 & 23.981 & 0.169 & 338.5 & 0.849 & 23.962 & 0.170 & 335.5 \\
% %         0.849 & 23.939 & 0.171 & 261 & 0.849 & 23.971 & 0.171 & 280.75 \\
% %         0.846 & 23.961 & 0.178 & 200 & 0.848 & 23.966 & 0.175 & 219.25 \\
% %         0.839 & 23.799 & 0.192 & 152 & 0.844 & 23.936 & 0.187 & 153 \\
% %         0.818 & 23.404 & 0.232 & 86 & 0.829 & 23.848 & 0.220 & 76.75 \\
% %         0.794 & 23.069 & 0.574 & 47 & 0.810 & 23.559 & 0.251 & 45.25 \\
% %         0.767 & 22.655 & 0.310 & 25 & 0.780 & 22.919 & 0.294 & 23.375 \\
% %         0.731 & 21.902 & 0.354 & 12.65 & 0.761 & 22.511 & 0.319 & 14.75 \\
% %     \bottomrule
% %     \end{tabular}
% %     }
% %     \caption{Performance comparison between opacity aware pruning and gradient aware opacity pruning on Tanks\&Temples dataset. Memory size is in MBs.}
% %     \label{tab: gradient aware pruning}
% % \end{table*}



% \subsection{Gradient Aware Pruning}
% \label{sec: pruning}
% 3DGS typically necessitates several million Gaussians to adequately model a standard scene, each Gaussian entailing 59 parameters. This results in a storage size significantly larger than that of most NeRF methodologies, such as Mip-NeRF360~\cite{barron2022mip}, K-planes~\cite{fridovich2023k}, and InstantNGP~\cite{muller2022instant}. Such requirements render 3DGS inefficient for certain applications, particularly those involving edge devices. Our primary focus is on parameter reduction. In the original training process of 3DGS, Kerbl~\etal~\cite{kerbl20233d} pruned and densified Gaussians up to a specified number of iterations, with pruning based on a predetermined opacity threshold. However, if their opacity is low and so is its gradient, we can say they can be removed with little to no impact on the quality of the rendered scene. As such, we have 

% % \begin{equation}
% %     \label{eq: pruning}
% %     \boldsymbol{\Sigma}' = \begin{cases}\Sigma_i & \text { if } \left( \left|\Sigma_i\right|>\mathcal{Q}_{|\boldsymbol{\alpha}|}(\gamma)\right) \lor \left( \left|\Sigma_i\right| > \mathcal{Q}_{|\boldsymbol{\nabla\mathcal{L}}|}(\gamma) \right)
% %     \\ 0 & \text { otherwise, }\end{cases}
% % \end{equation}

% % \begin{equation}
% %     \label{eq: pruning}
% %     \boldsymbol{\Sigma}' = \begin{cases}\Sigma_i & \text { if } \left( \left|\Sigma_i\right|\geq \mathcal{Q}_{|\boldsymbol{\alpha}|}(\gamma)\right) \lor \left( \left|\Sigma_i\right| \geq \mathcal{Q}_{|\boldsymbol{\nabla\mathcal{L}}|}(\gamma) \right)
% %     \\ 0 & \text { if } \left( \left|\Sigma_i\right|<\mathcal{Q}_{|\boldsymbol{\alpha}|}(\gamma)\right) \land \left( \left|\Sigma_i\right| < \mathcal{Q}_{|\boldsymbol{\nabla\mathcal{L}}|}(\gamma) \right),
    
% %     \end{cases}
% % \end{equation}


% % \begin{equation}
% %     \label{eq: pruning}
% %     \boldsymbol{\Sigma}' = \begin{cases}\Sigma_i & \text { if } \left( \left|\Sigma_{i}\left(\alpha \right)\right|\geq \mathcal{Q}_{|\boldsymbol{\Sigma_{i}\left(\alpha \right)}|}(\gamma)\right) \lor \left( \left|\nabla\Sigma_i\right| \geq \mathcal{Q}_{|\boldsymbol{\nabla\Sigma^i}|}(\gamma) \right)
% %     \\ 0  & \text { otherwise, }
    
% %     \end{cases}
% % \end{equation}
% \vspace{-5pt}
% \begin{equation}
%     \label{eq: pruning}
%     \boldsymbol{\Sigma}' = \begin{cases}
%      \Sigma_i & \text{if } \left[\left|\Sigma_i^\alpha\right|\geq \mathcal{Q}_{|\boldsymbol{\Sigma^\alpha}|}(\gamma_{\text{iter}})\right] \lor    \left[ \left|\nabla\Sigma_i\right| \geq \mathcal{Q}_{|\boldsymbol{\nabla\Sigma}|}(\gamma_{\text{iter}}) \right] \\
%     0  & \text{otherwise,}
%     \end{cases}
% \end{equation}



% \noindent where $\Sigma_i^\alpha$ denotes the $\alpha$ value of the $i$-th Gaussian, and $\nabla\Sigma_i$ denotes the gradient for the $i$-th Gaussian, $\mathcal{Q}_{|\boldsymbol{\Sigma^\alpha}|}(.)$ represents the quantile function for the opacity, $\mathcal{Q}_{|\boldsymbol{\nabla\Sigma}|}(.)$ is the quantile function for the gradients of the Gaussians, and $\gamma \in [0, 1]$ denotes the fraction of Gaussians to be removed. 
% %Through \eqref{eq: pruning}, we generate masks based on opacity and gradient separately and subsequently apply pruning solely on those Gaussians for which both masks evaluate to True. At a glance, to prune a specific Gaussian, it is necessary for both its opacity and gradient values to fall below the quantile threshold defined by $\gamma$. 
% This pruning process, along with periodic fine-tuning, not only improves performance but evidently results in substantial compression gains.

% %where $\mathcal{Q}_{|\boldsymbol{\alpha}|}(\cdot)$ represents the quantile function for the opacity of the Gaussians, while $\mathcal{Q}_{|\boldsymbol{\nabla\mathcal{L}}|}(.)$ signifies the quantile function for the gradients. $\gamma \in [0, 1]$ denotes the fraction of Gaussians to be removed. Utilizing the above \cref{eq: pruning}, we generate masks based on opacity and gradient separately and subsequently apply pruning solely on those Gaussians for which both masks evaluate to True. Put simply, to prune a specific Gaussian, it is necessary for both its opacity and gradient values to fall below the quantile threshold defined by $\gamma$. This pruning process, along with periodic fine-tuning, not only improves performance but also results in substantial compression gains.

% %where $\mathcal{Q}_{|\boldsymbol{\alpha}|}(\cdot)$ denotes the quantile function for the opacity of the Gaussians, with $\gamma \in [0, 1]$ representing the fraction of Gaussians to be removed. This pruning process, along with periodic fine-tuning, not only improves performance but also results in substantial compression gains.

% The iterative pruning and fine-tuning approaches enable the removal of redundant Gaussians while refining the remaining ones to better capture scene details compared to the baseline. Prior research in scene rendering has demonstrated that a gradual iterative pruning strategy can yield significantly sparser models while preserving high fidelity~\cite{deng2023compressing}. However, the impact of such an approach on 3DGS models yet remains unclear. We speculate that by gradually pruning the model over a specified number of iterations $t$ and aiming for a target sparsity $\gamma_{\text{target}}$, we can achieve improved results through a sparsification process applied to the 3DGS model: at every iteration, we apply the sparsification
% \begin{equation}
%     \gamma_{\text{iter}} = 1 - (1-\gamma_{\text{target}})^{\frac{1}{t}}.
% \end{equation}
% \noindent Our approach is based on two key factors. First, during the fine-tuning stage following pruning, the covariance $\Sigma$ is adjusted to minimize rendering loss, leading to higher values for solid surfaces and lower values for semi-transparent artifacts, which can be subsequently removed in the next iteration (which will be empirically observed in Fig.~\ref{fig: iterative vs one-shot}c). Second, the gradual iterative process helps prevent the optimization algorithm from converging to sub-optimal local minima (according to empirical evidence discussed in Sec.~\ref{sec:abl}). Hence, it is crucial to initiate the process with an overparametrized yet well-performing model. Similar observations can be drawn from traditional deep learning literature~\cite{blalock2020state, woodworth2020kernel}. In the next section, we will present a quantitative analysis of typical benchmarks employed for 3DGS.

% %%%% Results section starts here
% % \begin{figure}
% % \includegraphics[width=0.85\linewidth]{Figures/Gradient Aware.pdf}
% %     \centering
% %     \caption{The graph illustrates the performance-size trade-off obtained through opacity-aware pruning and gradient-aware opacity pruning on the Tanks\&Temple dataset. Both methods demonstrate considerable enhancements in performance and compression compared to the 3DGS-30k and 3DGS-7k baselines. Notably, gradient-aware pruning exhibits substantial performance improvement at lower compression rates.}
% %     \label{fig: gradient aware}
% %     \vspace{-0.4cm}
% % \end{figure}

% % \begin{table*}[ht]
% %     \caption{Performance comparison using gradient-aware iterative pruning with different pruning levels defined by $\gamma$ against 3DGS-30k, 3DGS-7k baselines, and opacity-based iterative pruning. $^*$Reproduced using official code. $^\dag$ Reported from~\cite{kerbl20233d}. Memory size is in MBs.
% %     %Comparison of performance using opacity-aware iterative pruning with different pruning levels defined by $\gamma$ against 3DGS-30k and 3DGS-7k baselines. $^*$Reproduced using official code. $^\dag$ Reported from \cite{kerbl20233d}. Memory size is in MBs.
% %     %Comparison of performance using opacity-aware iterative pruning with different pruning levels defined by $\gamma$ against 3DGS-30k and 3DGS-7k baselines. $^*$Reproduced using official code. $^\dag$ Reported from \cite{kerbl20233d}. Memory size is in MBs
% %     }
% %     \label{tab:pruning_comp}
% %     \centering
% %     \resizebox{\textwidth}{!}{
% %     \begin{tabular}{l|c|cccc|cccc|cccc}
% %     \toprule
% %       &   & \multicolumn{4}{c}{Mip-NeRF360} & \multicolumn{4}{c}{Tanks\&Temples} & \multicolumn{4}{c}{Deep Blending} \\
% %     \textbf{Model} & \textbf{$\boldsymbol{\gamma}$} & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\downarrow$ & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\downarrow$ & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\downarrow$ \\
% %     \midrule
    
% %    3DGS-7k$^\dag$ & -   & 0.770 & 25.60 & 0.279 & 523.00 &0.767 & 21.20 & 0.280 & 270.00 & 0.875 & 27.78 & 0.317 & 386.00 \\
% %     3DGS-30k$^\dag$ & -     & 0.815 & 27.21 & 0.214 &    734.00   & 0.841 & 23.14 & 0.183 &  411.00  & 0.903 & 29.41 & 0.243 & 676.00 \\
% %     3DGS-7k$^*$   & -    & 0.765 & 25.88 & 0.288 & 541.70  & 0.777 & 21.66 & 0.266 & 298.00 &  0.876 & 28.26 & 0.312 & 410.50  \\
% %     3DGS-30k$^*$ & -     & 0.812 & 27.46 & 0.221 & 763.40  & 0.845 & 23.69 & 0.178 & 435.50 & 0.899 & 29.51 & 0.246 & 664.50 \\
% % \midrule
% %     \multirow{8}{*}{\begin{tabular}{@{}p{2cm}@{}}3DGS-Opacity Based \\ Pruning\end{tabular}} & 0.025 & 0.813 & 27.58 & 0.217 & 592.22 & 0.849 & 23.98 & 0.169 & 338.50 & 0.894 & 29.27 & 0.248 & 516.00 \\
% %     & 0.050 & 0.813 & 27.56 & 0.220 & 449.11 & 0.849 & 23.94 & 0.171 & 261.00 & 0.894 & 29.27 & 0.250 & 398.00 \\
% %     & 0.075 & 0.809 & 27.47 & 0.231 & 344.00 & 0.846 & 23.96 & 0.178 & 200.00 & 0.895 & 29.27 & 0.252 & 305.00 \\
% %     & 0.100 & 0.799 & 27.25 & 0.250 & 261.78 & 0.839 & 23.80 & 0.192 & 152.00 & 0.894 & 29.22 & 0.259 & 232.00 \\
% %     & 0.150 & 0.762 & 26.46 & 0.304 & 148.00 & 0.818 & 23.40 & 0.232 & 86.00 & 0.888 & 28.96 & 0.279 & 131.00 \\
% %     & 0.200 & 0.725 & 25.66 & 0.353 & 80.89 & 0.794 & 23.07 & 0.574 & 47.00 & 0.883 & 28.66 & 0.295 & 72.00 \\
% %     & 0.250 & 0.692 & 24.98 & 0.394 & 42.78 & 0.767 & 22.66 & 0.310 & 25.00 & 0.877 & 28.20 & 0.310 & 38.00 \\
% %     & 0.300 & 0.659 & 24.26 & 0.430 & 22.14 & 0.731 & 21.90 & 0.354 & 12.65 & 0.869 & 27.69 & 0.328 & 19.00 \\
% % \midrule
% %     \multirow{8}{*}{\begin{tabular}{@{}p{2cm}@{}}3DGS-Gradient Aware \\ Pruning\end{tabular}} & 
% %     0.225 & 0.813 & 27.60 & 0.217 & 543.44 & 0.849 & 23.96 & 0.170 & 335.50 & 0.894 & 29.28 & 0.248 & 534.00 \\
% % & 0.275 & 0.814 & 27.60 & 0.219 & 464.33 & 0.849 & 23.97 & 0.171 & 280.75 & 0.894 & 29.26 & 0.248 & 481.50 \\
% % & 0.325 & 0.813 & 27.60 & 0.223 & 386.11 & 0.848 & 23.97 & 0.175 & 219.25 & 0.895 & 29.29 & 0.249 & 416.00 \\
% % & 0.375 & 0.810 & 27.56 & 0.231 & 311.78 & 0.844 & 23.94 & 0.187 & 153.00 & 0.895 & 29.29 & 0.250 & 339.00 \\
% % & 0.450 & 0.797 & 27.33 & 0.256 & 194.22 & 0.829 & 23.85 & 0.220 & 76.75 & 0.897 & 29.34 & 0.253 & 205.50 \\
% % & 0.500 & 0.776 & 26.92 & 0.288 & 119.44 & 0.810 & 23.56 & 0.251 & 45.25 & 0.898 & 29.37 & 0.258 & 118.50 \\
% % & 0.550 & 0.740 & 26.15 & 0.336 & 63.56 & 0.780 & 22.92 & 0.294 & 23.38 & 0.896 & 29.16 & 0.269 & 59.00 \\
% % & 0.600 & 0.690 & 25.03 & 0.394 & 29.22 & 0.761 & 22.51 & 0.319 & 14.75 & 0.887 & 28.62 & 0.293 & 25.50 \\
% %     \bottomrule


    
% %     \end{tabular}
% %     }
% % \end{table*}


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{Figures/Gradient Aware Comparison_updated.pdf}
%     \vspace{-10pt}
%     \caption{The graph depicts the trade-off between performance and size when utilizing Trimming the Fat (gradient-aware iterative pruning) compared to the 3DGS-30k and 3DGS-7k baselines as well as opacity-based pruning on the Mip-NeRF360, Tanks\&Temple, and Deep Blending datasets.}
%     \label{fig: comparison}
% \end{figure*}

% % \begin{wrapfigure}{r}{0.5\textwidth}
% % \centering
% % \vspace{-0.4cm}
% % \includegraphics[width=0.9\linewidth]{Figures/FPS Comparison.pdf}
    
% %     \caption{\salman{The graph illustrates the performance-size trade-off achieved by our method compared to the pruning approach proposed in Compact 3D~\cite{lee2023compact} on the Tanks\&Temple and Mip-NeRF360 datasets.}}
% %     \label{fig: FPS}
% %     \vspace{-0.4cm}
% % \end{wrapfigure}

% % \begin{wrapfigure}{r}{0.5\textwidth}
% % \centering
% % \vspace{-0.4cm}
% % \includegraphics[width=0.9\linewidth]{Figures/Pruning vs 3DCompact.pdf}
    
% %     \caption{\salman{The graph illustrates the performance-size trade-off achieved by our method compared to the pruning approach proposed in Compact 3D~\cite{lee2023compact} on the Tanks\&Temple and Mip-NeRF360 datasets.}}
% %     \label{fig: pruning vs 3DCompact}
% %     \vspace{-0.4cm}
% % \end{wrapfigure}

% % \begin{figure}[!htb]
% %     \centering
% %     \begin{minipage}[t]{0.22\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{Figures/Tanks and Temple FPS.pdf}
% %         \caption{\salman{The graph illustrates the effectiveness of our proposed method in enhancing the FPS of 3DGS.}}
% %         \label{fig: FPS}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.22\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{Figures/Tanks and Temple vs Compact3D.pdf}
% %         \caption{\salman{The graph illustrates the performance-size trade-off achieved by our method compared to the pruning approach proposed in Compact 3D~\cite{lee2023compact} on the Tanks\&Temple and Mip-NeRF360 datasets.}}
% %         \label{fig: pruning vs 3DCompact}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.22\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{Figures/Tanks and Temple vs Compact3D.pdf}
% %         \caption{\salman{The graph illustrates the performance-size trade-off achieved by our method compared to the pruning approach proposed in Compact 3D~\cite{lee2023compact} on the Tanks\&Temple and Mip-NeRF360 datasets.}}
% %         \label{fig: pruning vs 3DCompact}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.22\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{Figures/Tanks and Temple vs Compact3D.pdf}
% %         \caption{\salman{The graph illustrates the performance-size trade-off achieved by our method compared to the pruning approach proposed in Compact 3D~\cite{lee2023compact} on the Tanks\&Temple and Mip-NeRF360 datasets.}}
% %         \label{fig: pruning vs 3DCompact}
% %     \end{minipage}
% % \end{figure}


% \begin{figure*}[t]
% \includegraphics[width=0.85\linewidth]{Figures/mip-nerf-visual.pdf}
%     \centering
%     \vspace{-5pt}
%     \caption{Qualitative comparison of the garden scene at various pruning levels ($\gamma$) using gradient-aware iterative pruning. Our proposed method demonstrates substantially higher compression rates compared to both baselines while maintaining similar visual quality.}
%     \label{fig: Pruning-Comparison-1}
%     %\vspace{-0.4cm}
% \end{figure*}




% \section{Experiments and Results}
% %\vspace{-0.2cm}
% In this section, we present our empirical findings on commonly recognized benchmarks within the 3DGS community. We begin by detailing the implementation of our approach, followed by an outline of the benchmarked datasets and the evaluation metrics employed (Sec.~\ref{sec:idf}). Subsequently, we discuss both qualitative and quantitative results (Sec.~\ref{sec:res}), providing as well an ablation study (Sec.~\ref{sec:abl}).

% \subsection{Implementation Details}
% \label{sec:idf}
% %In all our experiments, we utilize the publicly available official code repository of 3DGS \cite{kerbl20233d} without making any alterations to the hyperparameters used for training, ensuring consistency with the original 3DGS model.
% In all our experiments, we use the publicly available official code repository of 3DGS~\cite{kerbl20233d}, adhering to the recommended hyperparameter settings used for training to maintain consistency with the original 3DGS model. We initiate the pruning process with the optimized Gaussians trained for 30,000 iterations, employing pruning with %$\gamma = [0.225, 0.275, 0.325, 0.375, 0.45, 0.5, 0.55, 0.6]$
% $\gamma_{\text{iter}}\in[0.225,0.6]$, as described in \eqref{eq: pruning}.  Iterative pruning with the same $\gamma_{\text{iter}}$ value is applied after every 500 iterations until reaching 35,000 iterations (commencing from 30,000 iterations), followed by further fine-tuning for 10,000 iterations. For all our experiments, pruning and fine-tuning consistently yield significantly improved compression-performance trade-offs. Additionally, $\lambda= 0.2$ is employed consistently across all our experiments. 

% %For all our experiments, we employ the publicly available official code repository of 3D Gaussian Splat \cite{kerbl20233d}, without modifying the hyperparameters used for training compared to the original 3D Gaussian Splat model. We begin the pruning process with the optimized Gaussians trained for 30,000 iterations, applying pruning using \eqref{eq: pruning} with $\gamma$, where $~{\gamma = [0.225, 0.275,0.325,0.375,0.45,0.5,0.55,0.6]}$. The model undergoes sequential pruning with the same $\gamma$ value after every 1000 iterations until reaching 40,000 iterations (starting from 30,000 iterations), followed by further finetuning for 20,000 iterations. In most experiments, pruning and finetuning result in superior performance compared to the baseline.
% \noindent\textbf{Datasets.} We assess the efficacy of our pruning approach across diverse scenes, encompassing environments from the Mip-Nerf360~\cite{barron2022mip} indoor and outdoor datasets, alongside two scenes sourced from the Tanks\&Temples~\cite{knapitsch2017tanks} and Deep Blending~\cite{hedman2018deep} datasets, akin to the scenes examined in the original 3DGS work~\cite{kerbl20233d}.

% \noindent\textbf{Evaluation.} To ensure a fair comparison, we adhere to the same train-test split utilized in Mip-Nerf360~\cite{barron2022mip} and 3DGS~\cite{kerbl20233d}. %Moreover, we include our reproduced metrics for 3DGS, as we observed slightly enhanced results compared to those reported in~\cite{kerbl20233d} for certain scenes when executing their code ourselves. 
% Our evaluation encompasses standard metrics like SSIM, PSNR, and LPIPS, alongside the average memory consumption across all datasets.


% \subsection{Results}
% \label{sec:res}
% \subsubsection{Quantitative Comparison} 
% \textbf{Trimming the Fat.} We conduct a comparative analysis between our method, the 3DGS-30k, and 3DGS-7k baselines, along with an opacity-based pruning approach that removes gradient information from \eqref{eq: pruning}. As illustrated in Fig.~\ref{fig: comparison}, we examine the trade-off in compression performance across benchmark datasets. Across all the datasets, Gaussian splats can be pruned by up to 4$\times$, showcasing improved or similar performance compared to the baseline. Notably, even at significantly high pruning levels, where the average scene size is less than 25MB, our proposed pruning technique maintains comparable or even superior performance to that of the 3DGS-7k variant, achieving compression rates of up to 24$\times$ on average. This is realized without the need for any additional end-to-end compression pipeline integration, highlighting the standalone scalability of our proposed approach. 
% %We compare our method with the 3DGS-30k and 3DGS-7k baselines, as well as with an opacity-based pruning approach, in which the gradient information from \cref{eq: pruning} is removed. Figure~\ref{fig: comparison} illustrate the tradeoff in compression performance across benchmark datasets. For the Tanks\&Temples and Mip-NeRF360 datasets, Gaussian splats can be pruned by up to 4$\times$ with improved or similar performance compared to the baseline. However, in the Deep Blending dataset, our best pruning model results in a negligible loss of about 0.07 PSNR. It is worth noting that a PSNR difference of 0.5 is imperceptible to the human eye \cite{salomon2010handbook}. Similarly, for Deep Blending, Gaussian splats can be pruned by more than 4$\times$ without a drop in performance. Further compression reveals information loss, yet our method maintains performance better/ similar to the 3DGS-7k baseline, achieving compression rates of up to 24$\times$ on average.

% Opacity-based pruning exhibits similar performance to gradient-aware pruning at small pruning thresholds. However, the performance difference becomes more pronounced at higher compression rates, as evident from the results in Fig.~\ref{fig: comparison}. Incorporating gradient information leads to additional performance improvements in pruning. This enhancement arises because certain scene features (sky, glass, etc.) may have low opacity but are still crucial for overall scene rendering. By considering gradient information, we ensure that only Gaussians containing unimportant features are pruned. Our proposal of incorporating information on the gradient shows its prominent effectiveness at higher pruning rates. For a more detailed comparison please refer to the supplementary material.

% \begin{figure}
%     \begin{tabular}{@{}c@{}c@{}c@{}}
%         \bmvaHangBox{\includegraphics[width=0.3\columnwidth]{Figures/One Shot Pruning vs Iterative Pruning (1).pdf}}&
%         \bmvaHangBox{\includegraphics[width=0.3\columnwidth]{Figures/Tanks and Temple FPS.pdf}}&
%         \bmvaHangBox{\includegraphics[width=0.4\columnwidth]{Figures/b_p_opacity (1).pdf}}\\
%         (a)&(b)&(c)\\
%     \end{tabular}
%     \vspace{-10pt}
%     \caption{Trade-off between performance and size through iterative pruning and one-shot pruning techniques (a) and in terms of FPS on the Tanks\&Temples dataset (b), and opacity distribution before and after pruning for the \texttt{truck} scene (c).}% Both approaches exhibit significant improvements in performance and compression compared to the 3DGS-30k and 3DGS-7k baselines.}
%     \label{fig: iterative vs one-shot}
% \end{figure}
% %\begin{wrapfigure}{r}{0.4\textwidth}
% %\centering
% %\vspace{-0.4cm}

% %    
% %\end{wrapfigure}
% \noindent
% \textbf{Trimming the Fat with end-to-end compression.}
% Our proposed pruning methodology can act as a plug-and-play with various end-to-end compression techniques for 3DGS. When integrated with the method proposed by Niedermayr~\emph{et~al.}~\cite{niedermayr2023compressed}, we achieve state-of-the-art compression performance. Niedermayr's approach begins with a pre-trained Gaussian as the foundation of its compression process. We substitute this pre-trained Gaussian with our pruned Gaussian and apply the end-to-end compression procedure. This combination results in 50$\times$ compression compared to the baseline, while maintaining comparable performance. Moreover, we achieve 2$\times$ compression with improved performance compared to Niedermayr's original approach, as demonstrated in Table~\ref{tab:compression_comp}. %For initialization of our compression pipeline, we employ pre-trained scenes pruned at specific thresholds: $\gamma = 0.325$ for the Mip-NeRF360 dataset, $\gamma = 0.425$ for Tanks\&Temple, and $\gamma = 0.475$ for Deep Blending.

% %Table \ref{tab:pruning_comp} compares our method with the 3DGS-30k and 3DGS-7k baselines, while the \cref{fig: comparison} illustrates the tradeoff in compression performance across benchmark datasets. In the Tanks\&Temples and Mip-NeRF360 datasets, Gaussian splats can be pruned by up to half with better performance than the baseline. However, for the Deep Blending dataset, pruning results in an indiscernible loss of about 0.25 PSNR. It is important to note that a PSNR difference of 0.5 is indistinguishable to the human eye \cite{salomon2010handbook}. Similarly, for Deep Blending, Gaussian splats can be pruned by more than 50\% without a drop in performance. Information loss becomes evident with further compression. Nevertheless, even with very high compression rates, our method maintains performance similar to the 3DGS-7k baseline, achieving compression rates of up to 24$\times$ on average.
% \vspace{-0.4cm}
% \subsubsection{Qualitative Comparison} We present visualizations of the \texttt{garden} scene from the Mip-NeRF360 dataset, which typically demands substantial memory resources. In Fig.~\ref{fig: Pruning-Comparison-1} we showcase the visualizations of test set images at various pruning levels denoted by $\gamma_{\text{iter}}$. Our gradient-aware iterative pruning pipeline demonstrates significant compression rates while maintaining comparable visual quality. Specifically, our method compresses the Gaussian splats by approximately $4\times$ with visual quality akin to 3DGS-30K. Moreover, with $\gamma_{\text{iter}}=0.60$, our method achieves a compression ratio of approximately 25$\times$ while preserving visual quality comparable to 3DGS-7K. For additional visualizations, please refer to the supplementary material.



% %We present visualizations of scenes from the Tanks \& Temples, Mip-NeRF360, and Deep Blending datasets, all of which require substantial memory resources on average. In \cref{fig: Pruning-Comparison-1,fig: Pruning-Comparison-2,fig: Pruning-Comparison-3}, we illustrate the visualizations of test set images at various pruning levels indicated by $\gamma$. Our gradient-aware iterative pruning pipeline achieves noteworthy compression rates while maintaining comparable visual quality. Across all scenes depicted in the \cref{fig: Pruning-Comparison-1,fig: Pruning-Comparison-2,fig: Pruning-Comparison-3}, our method compresses the Gaussian splats by approximately $4\times$ with visual quality similar to 3DGS-30K. Furthermore, with $\gamma=0.60$, our method achieves an average compression ratio of approximately 12$\times$ while preserving visual quality comparable to 3DGS-7K.

% \subsection{Ablation Study}
% \label{sec:abl}
% \textbf{FPS Gain with Trimming the Fat.} Our novel pruning approach significantly enhances the FPS rate of 3DGS. On the Tanks\&Temples dataset, our method achieves an FPS of over 600+ all while maintaining SOTA performance as shown in~Fig.~\ref{fig: iterative vs one-shot}b. The renderings were performed using an RTX-3090, and the final FPS reported were averaged over three separate runs. These findings demonstrate the scalability of our proposed method.% for low-powered edge devices.

% % \textbf{Trimming the Fat vs Compact3D~\cite{lee2023compact}.} \salman{Fig.~\ref{fig: iterative vs one-shot}b depicts a comparison of PSNR and Gaussian counts between our proposed approach and Compact 3D using the Tanks\&Temples dataset. The results unequivocally highlight the superior performance of our method, demonstrating its capability to significantly reduce the number of Gaussians while maintaining baseline performance levels. These findings emphasize the effectiveness of our pruning technique and its potential to advance or replace existing compression methodologies for 3DGS.} 

% %Figure~\ref{fig: pruning vs 3DCompact} illustrate the comparison of PSNR and the number of Gaussians between our approach and Compact 3D for the Tanks\&Temple dataset. The Fig.~\ref{fig: pruning vs 3DCompact} unequivocally demonstrate the superiority of our proposed method for the benchmark dataset. The results underscore the significance of our pruning approach compared to existing methods in the literature~\cite{lee2023compact}.}

% \noindent\textbf{Why 3D Prior for Pruning is important?}
% To assess the significance of a 3D prior in the pruning process, we modified the original training protocol introduced by Kerbl~\etal~\cite{kerbl20233d}. In their methodology, Gaussians are pruned and densified up to a specified iteration count (15k), employing an opacity threshold for pruning. Our modification involved halting the densification phase at the same iteration count (15k) but extending the pruning phase for an additional 10k iterations. Subsequently, the model underwent further fine-tuning for an additional 5k iterations to generate the final scene. The findings are outlined in Fig.~\ref{fig: iterative vs one-shot}a, indicating that even with a reduced pruning threshold, achieving convergence without a robust 3D prior remains challenging for a 3DGS model.%To assess the significance of a 3D prior in the pruning process, we adapted the original training protocol introduced by Kerbl et al.~\cite{kerbl20233d}. In their methodology, Kerbl et al. pruned and refined Gaussians up to a specified iteration count (15k), employing an opacity threshold for pruning. Our modification involved halting the refinement phase at the same iteration count (15k) but extending the pruning phase for an additional 10k iterations. Subsequently, the model underwent further fine-tuning for an additional 5000 iterations to generate the final scene. The findings are outlined in the~\cref{tab:3D-prior}, indicating that even with a reduced pruning threshold, achieving convergence without a robust 3D prior remains challenging for a 3DGS model.}

% \noindent\textbf{Why Pruning is effective?}
% Our proposed pruning technique achieves compression ratios of up to $4\times$ without compromising performance compared to the 3DGS baseline. The efficacy of our approach lies in its ability to effectively eliminate redundant Gaussians. As depicted in Fig.~\ref{fig: iterative vs one-shot}c, the opacity distribution before and after pruning for the \texttt{truck} changes significantly. For the baseline 3DGS, the majority of opacity values are very low, indicating minimal contribution to scene reconstruction. However, through post-hoc pruning, a significant proportion of opacity values become notably higher, indicating that a more solid geometry is learned by the model.

% \noindent\textbf{One Shot Pruning vs Iterative Pruning.}
% We also explored the impact of one-shot pruning in comparison to iterative pruning, in terms of model size, showcased in Fig.~\ref{fig: iterative vs one-shot}a. For one-shot pruning, we utilized the pre-trained 3DGS-30k model, performed the pruning process once, and then fine-tuned the model for 30k iterations. Both gradient-aware and opacity-based iterative pruning consistently outperformed the one-shot pruning method: our results demonstrate that gradual pruning enables the model to better adapt to the scene compared to one-shot pruning. %  The memory size reflects the effectiveness of pruning on the 3DGS, as depicted in Fig.~\ref{fig: iterative vs one-shot}a. 

% %We explored the impact of one-shot pruning in comparison to iterative pruning. Our results demonstrate that gradual pruning enables the model to better adapt to the scene compared to one-shot pruning. For one-shot pruning, we utilized the pretrained 3DGS-30k model, performed the pruning process once, and then fine-tuned the model for 30k iterations. Table \ref{tab:one-shot-pruning_comp} presents a comprehensive comparison between one-shot pruning and iterative pruning on the Tanks\&Temples dataset, while the compression performance tradeoff is visualized in \cref{fig: iterative vs one-shot}. The memory size reflects the effectiveness of pruning on the 3DGS, as depicted in both Table \ref{tab: one-shot-pruning_comp} and \cref{fig: iterative vs one-shot}.


% % \subsubsection{Lottery Ticket for the Gaussian Splats?}\enzo{this whole section lacks the experiment outcome!} We investigated the potential presence of a ``lottery ticket'' phenomenon~\cite{frankle2018lottery} for Gaussian splats. To test this hypothesis, we took an already pruned set of Gaussian splats from the Tanks\&Temples dataset and randomly reinitialized all learnable features, including spherical harmonics (SH) features, opacity, scale, and rotation. Subsequently, we attempted to train these Gaussian splats for 30,000 iterations, but they failed to converge. This experiment underscores the necessity of having a learned 3D prior to which redundant information can be pruned. It highlights the difficulty of training Gaussian splats with the minimum number of Gaussians without any prior information from the 3D scene.




% %\noindent\textbf{Gradient Aware Opacity Pruning:}
% %We also examined the influence of gradient information on opacity-aware pruning. In this analysis, we utilized the same threshold value, denoted by $\gamma$, for both calculating the mask based on gradient and opacity. The approach involved generating masks based on opacity and gradient separately and then pruning only those Gaussians for which both masks evaluated to true. In simpler terms, to prune a specific Gaussian, it was required that both its opacity and gradient values fell below the quantile threshold defined by $\gamma$. The results obtained from the Tanks\&Temples dataset are presented in both the Table~\ref{tab: gradient aware pruning} and \cref{fig: gradient aware}. The findings indicate that incorporating gradient information leads to further performance improvements in pruning. This enhancement stems from the fact that certain scene features may possess low opacity but are still crucial for overall scene rendering. By considering gradient information, we ensure that only Gaussians containing unimportant features are pruned. This effectiveness becomes more pronounced at higher pruning rates.

% %\vspace{-0.2cm}

% \begin{table}[t]
%     \caption{Performance and compression comparison of 3DGS baseline, end-to-end compression~\cite{niedermayr2023compressed}, and our proposed method with the reference end-to-end compression method. Comp. stands for compression rate. $^\dag$ Reported from~\cite{niedermayr2023compressed}. }
%     \label{tab:compression_comp}
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|ccccc|ccccc|ccccc}
%     \toprule
%       &  \multicolumn{5}{c}{3D Gaussian Splatting$^\dag$} & \multicolumn{5}{c}{End to End Compression~\cite{niedermayr2023compressed}$^\dag$} & \multicolumn{5}{c}{Our's Trimming the Fat with End to End Compression} \\
%     \textbf{Dataset} & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\downarrow$ & \textbf{Comp.}$^\uparrow$ & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} &  \textbf{Mem}$^\downarrow$ &  \textbf{Comp.}$^\uparrow$ & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\uparrow$ & \textbf{Comp.}$^\uparrow$\\
%     \midrule
    
%    Mip-NeRF360 & 0.812 & 27.287 & 0.220 & 795.263 & 1$\times$ &  0.801 & 26.981 & 0.238 & 28.803 & 26.230$\times$ & 0.798 & 27.130 & 0.248 & 20.057 & 39.650$\times$ \\
%    Tanks\&Temples & 0.838  & 23.355 & 0.186 & 421.906 &   1$\times$ &  0.832 & 23.343 & 0.194 & 17.282 &  23.260$\times$  & 0.831 & 23.689 & 0.210 & 8.555 & 49.317$\times$ \\
%    Deep Blending  & 0.898  & 29.432  & 0.246 & 703.772 & 1$\times$ & 0.898 & 29.381   & 0.253  & 25.299 & 27.816$\times$ &  0.897 & 29.425 & 0.267 & 12.494 & 56.329$\times$ \\

%     \bottomrule
%     \end{tabular}



    
%     }
% \end{table}


% % \begin{table}[t]
% %     \caption{\salman{Comparison between the baseline 3DGS-30k model, its variant with additional pruning, and the proposed method.}}
% %     \label{tab:3D-prior}
% %     \centering
% %     \resizebox{\textwidth}{!}{
% %     \begin{tabular}{l|cccc|cccc}
% %     \toprule
% %       &  \multicolumn{4}{c}{Train} & \multicolumn{4}{c}{Truck} \\
% %      Method & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\downarrow$ & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} &  \textbf{Mem}$^\downarrow$\\
% %     \midrule
% % 3DGS-30k Baseline & 0.710 & 19.481 & 0.331 & 257 & 0.878 & 25.313 & 0.147 & 614 \\
% % 3DGS-30k with Additional Pruning & 0.752 & 19.887 & 0.287 & 134 & 0.856 & 24.364 & 0.192 & 525 \\
% % Gradient Aware Pruning & 0.804 & 22.449 & 0.234 & 64 & 0.867 & 25.360 & 0.182 & 126 \\

% %     \bottomrule
% %     \end{tabular}
% %     }
% % \end{table}



% %  \begin{figure*}[t]
% %     \centering
% %     \includegraphics[width=1.0\linewidth]{Figures/Gradient Aware Comparison.pdf}
% %     \caption{The graph depicts the trade-off between performance and size when utilizing gradient-aware iterative pruning compared to the 3DGS-30k and 3DGS-7k baselines as well as opacity-based pruning on the Mip-NeRF360, Tanks\&Temple, and Deep Blending datasets.}
% %     \label{fig: comparison}
% % \end{figure*}

% \vspace{-0.2cm}

% \section{Conclusion}
% In this work, we presented a gradient-aware iterative pruning technique for 3D Gaussian splats named after ``Trimming the fat''. Our method effectively scales down Gaussian splats by a factor 4$\times$ without sacrificing generative quality. Particularly at higher pruning levels, our proposed method achieves compression ratios of approximately 25$\times$ and achieves up to 600~FPS with minimal impact on generative performance across established benchmark datasets. The resulting highly compressed point clouds can be seamlessly transmitted over networks and utilized on resource-constrained devices, offering potential applications in mobile VR/AR and gaming. Future research directions include investigating the integration of quantization-aware training methods to further improve the compressibility of 3DGS.
% %We have presented an opacity-aware iterative pruning technique for 3D Gaussians. Our method effectively prunes Gaussian splats by half without sacrificing information, achieving compression ratios of approximately 25$\times$ with minimal impact on generative performance across established benchmark datasets. The significantly compressed Gaussian point cloud can be seamlessly streamed over networks and rendered on low-power devices, rendering it suitable for mobile VR/AR applications and games. Moving forward, we intend to explore the integration of gradient information to enhance the pruning pipeline further.




% \bibliography{main}
% \end{document}


==> main_2.tex <==
% \documentclass{bmvc2k}

% \usepackage{graphicx}
% \usepackage{cleveref}
% \usepackage{multirow}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{booktabs}
% \usepackage{wrapfig}
% \usepackage{enumitem}

% %% Enter your paper number here for the review copy
% % \bmvcreviewcopy{??}

% \title{Trimming the Fat: Efficient Compression of 3D Gaussian Splats through Pruning}

% % Enter the paper's authors in order
% % \addauthor{Name}{email/homepage}{INSTITUTION_CODE}
% \addauthor{Muhammad Salman Ali}{salmanali@khu.ac.kr}{1,2}
% \addauthor{Maryam Qamar}{maryamqamar@khu.ac.kr}{2}
% \addauthor{Sung-Ho Bae}{shbae@khu.ac.kr}{2}
% \addauthor{Enzo Tartaglione}{enzo.tartaglione@telecom-paris.fr}{1}

% % Enter the institutions
% % \addinstitution{Name\\Address}
% \addinstitution{
%  LTCI, Télécom Paris,\\ Institut Polytechnique de Paris, France
% }
% \addinstitution{
%  Kyung Hee University,\\ Republic of Korea
% }

% \runninghead{Ali et al.}{Efficient Compression of 3DGS through Pruning}

% % Any macro definitions you would like to include
% % These are not defined in the style file, because they don't begin
% % with \bmva, so they might conflict with the user's own macros.
% % The \bmvaOneDot macro adds a full stop unless there is one in the
% % text already.
% \def\eg{\emph{e.g}\bmvaOneDot}
% \def\Eg{\emph{E.g}\bmvaOneDot}
% \def\etal{\emph{et al}\bmvaOneDot}

% %-------------------------------------------------------------------------
% % Document starts here
% \begin{document}

% \maketitle
% \begin{abstract}
% %In recent times, the utilization of 3D models has gained traction, owing to the capacity for end-to-end training initially offered by Neural Radiance Fields and more recently by 3D Gaussian Splatting (3DGS) models. The latter holds a significant advantage by inherently facilitating rapid convergence during training and offering extensive editability. However, despite advancements, the literature still lacks exploration into the scalability of these models. In this study, we take the initial steps in addressing this gap showing an approach that enables both the memory and computational scalability of such models. Specifically, we propose an iterative pruning technique to eliminate redundant information encoded in the model. We show that a simple magnitude-based approach achieves subpar results when compared to a gradient-informed one, despite traditional pruning literature showing that not being the typical case. Our experimental findings on widely acknowledged benchmarks attest to the effectiveness of our approach, revealing that up to 75\% of the Gaussians can be removed while maintaining or even improving upon baseline performance. Given that the pruned Gaussians are entirely eliminated, this directly influences the scalability of the Gaussians, thus indicating the potential for widespread deployment, even on devices with limited resources. By integrating our pruning method with an end-to-end compression approach for 3D Gaussian Splatting (3DGS), we attain state-of-the-art compression performance. Our combined approach achieves compression rates of around 50$\times$, while preserving performance similar to the baseline model. We commit to release the code open-source upon acceptance of the article.
% In recent times, the utilization of 3D models has gained traction, owing to the capacity for end-to-end training initially offered by Neural Radiance Fields and more recently by 3D Gaussian Splatting (3DGS) models. The latter holds a significant advantage by inherently easing rapid convergence during training and offering extensive editability. However, despite rapid advancements, the literature still lives in its infancy regarding the scalability of these models. In this study, we take some initial steps in addressing this gap, showing an approach that enables both the memory and computational scalability of such models. Specifically, we propose ``Trimming the fat'', a post-hoc gradient-informed iterative pruning technique to eliminate redundant information encoded in the model. %We show that a simple magnitude-based approach achieves subpar results when compared to a gradient-informed one, despite traditional pruning literature showing that not being the typical case. 
% Our experimental findings on widely acknowledged benchmarks attest to the effectiveness of our approach, revealing that up to 75\% of the Gaussians can be removed while maintaining or even improving upon baseline performance. %By integrating our pruning method with an end-to-end compression approach for 3D Gaussian Splatting (3DGS), we attain state-of-the-art compression performance. 
% Our approach achieves around 50$\times$ compression while preserving performance similar to the baseline model, and is able to speed-up computation up to 600~FPS. We commit to release the code open-source upon acceptance of the article.
% \end{abstract}

% %-------------------------------------------------------------------------
% \section{Introduction}
% \label{sec:intro}
% \begin{figure}[t]%{r}{0.7\textwidth}
%     %\vspace{-10pt}
%     \centering
%     \includegraphics[width=0.7\linewidth]{Figures/Teaser_try_again1.pdf}
%     \caption{%Comparison of 3DGS-30k with Niedermayr's Compression, our pruning method, and their combination yields compelling results. Our pruning compresses scenes by up to 4.5$\times$ without sacrificing visual quality. It seamlessly integrates with any compression method. Combined with Niedermayr's approach, we achieve up to 60$\times$ compression with similar visual quality.
%     Vanilla 3DGS-30k VS our novel pruning approach applied with an end-to-end compression technique~\cite{niedermayr2023compressed}.% Our pruning method achieves scene compression of up to 7.5$\times$ without compromising visual fidelity, integrating smoothly with diverse compression methods. When paired with the Niedermayr et al. method~\cite{niedermayr2023compressed}, we achieve compression rates of up to 60$\times$ while preserving comparable visual quality.}
%     }
%     \label{fig:teaser}
%     %\vspace{-0.4cm}
% \end{figure}
% In the last few years, significant advancements have been made in radiance field methodologies for reconstructing 3D scenes using images captured from various viewpoints. The emergence of Neural Radiance Fields (NeRF) techniques has notably influenced the realm of 3D scene modeling and reconstruction~\cite{mildenhall2021nerf,huang2022stylizednerf}. The efficient generation of photo-realistic novel views from a given set of training images has become a focal point in computer vision research, with diverse applications~\cite{deng2023compressing}. NeRF's capability to distill the essence of a 3D object from its 2D representations, while maintaining compactness, underscores its impact and popularity in the literature~\cite{yu2021pixelnerf,kaya2022neural}.

% Despite its success, the traditional NeRF~\cite{mildenhall2021nerf} suffers from slow training and rendering speeds. To address this challenge, various approaches have been proposed, although they often entail compromises in rendered image quality~\cite{deng2023compressing}. Recent studies have turned to explicit scene representations, such as voxel-based~\cite{sun2022direct} or point-based~\cite{xu2022point} structures to enhance rendering efficiency. For instance, leveraging 3D voxel grids on GPUs alongside multi-resolution hash encoding of inputs led to consistent reductions in required operations and enabled real-time performance~\cite{muller2022instant}. Similarly, the most efficient radiance field solutions to date rely on continuous representations achieved through interpolating values stored in voxel~\cite{fridovich2022plenoxels}, hash grids~\cite{muller2022instant}, or points~\cite{xu2022point}. While the continuous nature of these methods aids optimization, the stochastic sampling necessary for rendering can incur computational overhead and introduce noise~\cite{kerbl20233d}.

% % \begin{wrapfigure}{r}{0.5\textwidth}
% %     \centering
% %     \includegraphics[width=0.99\linewidth]{Figures/teaser.pdf}
% %     \caption{Qualitative comparison of our proposed method and original 3DGS-30k. With our proposed method we can achieve compression rates of about $7.5\times$ with indiscernible loss in visual quality simply with proper pruning.}
% %     \label{fig:teaser}
% %     \vspace{-0.4cm}
% % \end{wrapfigure}

% A recent advancement in the field is the introduction of differentiable 3D Gaussian splatting (3DGS), which enables the generation of a sparse adaptive scene representation~\cite{kerbl20233d}. This representation can be rendered rapidly on the GPU, offering big speed improvements. 3DGS combines the best features of existing methods: leveraging a 3D Gaussian representation for scene optimization provides state-of-the-art visual quality and competitive training times while the tile-based splatting solution ensures real-time rendering at high quality for 1080p resolution across various datasets. Unlike NeRF methods, 3DGS simplifies training and rendering by projecting 3D Gaussians to the 2D image space and combines them with opacity using \emph{rasterization}, enabling real-time rendering on a single GPU. Furthermore, the explicit storage of scene structure in the parameter space allows for direct editing of the 3D scene. However, some challenges emerge when employing differentiable 3DGS, particularly in optimizing scenes with millions of Gaussians, which may require substantial storage and memory. While specialized pipelines demonstrate real-time performance on high-end GPUs, seamless integration into VR/AR environments or games remains a challenge, particularly when working alongside hardware rasterization of polygon models.

% In this paper, we aim to compress Gaussian splatting representations while preserving their rendering speed and quality, facilitating their application across diverse domains such as IoT devices with limited storage or memory. Our primary insight is that the learned 3DGS models exhibit over-fitting to the underlying scene, allowing for the removal or pruning of many Gaussians without sacrificing performance, particularly due to markedly lower opacity values. We start the training process with a pre-trained optimized Gaussian scene, iteratively pruning it based on opacity levels and gradient values, followed by fine-tuning to achieve superior performance-compression trade-off compared to the baseline optimized scene as showcased from Fig.~\ref{fig:teaser}. Our main contributions are the following.

% %We start the training process with a pre-trained optimized Gaussian scene, iteratively pruning it based on opacity levels and gradient values, followed by fine-tuning to achieve superior performance compared to the baseline optimized scene. Our main contributions are as follows:

% \begin{itemize}[noitemsep, nolistsep]
%     \item We build on top of the optimized 3DGS as a 3D prior for pruning, enabling the removal of redundant Gaussians while fine-tuning the remaining ones to accurately capture the scene features (Sec.~\ref{sec: pruning}). 
    
%     \item We observe that vanilla pruning is sub-optimal when compared to a gradient-informed approach and that pruning without such a prior fails. Besides, we showcase the compatibility with other compression pipelines, like~\cite{niedermayr2023compressed} (Sec.~\ref{sec:abl}).

%     \item With our proposed method, we achieve state-of-the-art performance even after pruning 50\% of the Gaussian splats, significantly enhancing the scalability of 3DGS (Sec.~\ref{sec:res}). Our compression pipeline achieves an enhanced balance between scene fidelity and compression, surpassing the baseline (Fig.~\ref{fig: Pruning-Comparison-1}). %To the best of our knowledge, our iterative pruning approach stands as the state-of-the-art: when integrated with the existing end-to-end compression approach~\cite{niedermayr2023compressed}, our method achieves a compression ratio of approximately 50$\times$, all while preserving performance metrics akin to those of the baseline (Sec.~\ref{sec:res}).
% \end{itemize}

% %Since the main focus of this work is on showing and discussing the contribution of pruning, although extra compression steps are possible (including vector quantization, entropy coding, Morton ordering etc.) we did not include or compare with them, as it stands out the scope of this work which is a study on the effect of proper pruning to compress 3DGS models.



% \section{Related Work}
% \label{sec:Related Work}
% In this section we first provide an overview of the most recent methods for novel view synthesis (Sec.~\ref{sec:nws}), then we discuss approaches for their compression (Sec.~\ref{sec:3dgs-compress}).

% \subsection{Novel View Synthesis}
% \label{sec:nws}
% Recent advancements in novel view synthesis have seen significant progress, with early techniques using CNNs to estimate blending weights or texture-space solutions~\cite{flynn2016deepstereo, hedman2018deep,riegler2020free,thies2019deferred}, albeit facing challenges with MVS-based geometry and temporal flickering. Volumetric representations, starting with Soft3D~\cite{penner2017soft} and employing deep learning with volumetric ray-marching~\cite{henzler2019escaping,sitzmann2019deepvoxels}, provided further advancements. Neural Radiance Fields (NeRFs)~\cite{mildenhall2021nerf} aimed to enhance synthesized views' quality but faced slow processing due to a large Multi-Layer Perceptron (MLP) backbone and dense sampling. Subsequent methods like Mip-NeRF360~\cite{barron2022mip} focused on balancing quality and speed, while recent advances prioritize faster training and rendering through spatial data structures, encodings, and MLP adjustments~\cite{chen2023mobilenerf,fridovich2022plenoxels,garbin2021fastnerf}. Notable methods such as InstantNGP~\cite{muller2022instant} leverage hash grids and occupancy grids for accelerated computation, while Plenoxels~\cite{fridovich2022plenoxels} rely on Spherical Harmonics for directional effects without neural networks. Despite these strides, challenges persist in NeRF methods regarding efficient coding for empty space, image quality, and rendering speed.

% In contrast, 3DGS achieves superior quality and faster rendering without implicit learning. However, its increased storage compared to NeRF methods poses limitations. Our approach aims to maintain the quality and speed of 3DGS while reducing model storage by applying pruning to Gaussian parameters.
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{Figures/3DGS-overview.pdf}
%     \caption{Overview of our pruning pipeline. From a pre-trained 3DGS-30k scene, we first iteratively prune it for a fixed number of iterations with subsequent fine-tuning. Then, we conduct further fine-tuning for 20,000 iterations to obtain our final optimized scene.}
%     \label{fig:overview}
% \end{figure*}
% %\subsection{NeRFs Compression}
% %\label{sec:compress}
% % Various methods have emerged to address the computational costs associated with NeRF's dense sampling of color values and opacity. These methods adopt different data structures such as trees~\cite{wang2022fourier, yu2021plenoctrees}, point clouds~\cite{peng2021shape,xu2022point}, and grids~\cite{chen2022tensorf, fridovich2022plenoxels, muller2022instant,sun2022direct} to efficiently represent 3D scenes and objects. Grid structures, for instance, enable training iterations to be completed in a matter of minutes, but they may require substantial memory due to their dense nature. To mitigate this, several approaches have focused on reducing the size of volumetric grids~\cite{chen2022tensorf,huang2022pref,takikawa2022variable}. Instant-NGP~\cite{muller2022instant} utilizes hash-based multi-resolution grids, while VQAD~\cite{takikawa2022variable} replaces the hash function with codebooks and vector quantization.  
% %  VQRF~\cite{li2023compressing} compresses volumetric grid-based radiance fields by adopting vector quantization. Additionally, frequency domain transformation~\cite{rho2023masked,zhao2023tinynerf}, and voxel pruning~\cite{deng2023compressing} have also been proposed to reduce the memory consumption of grid-based NeRFs. Despite these efforts, grid-based NeRF variants still have larger sizes compared to MLP-based methods.

% % Although dense voxel-based representations significantly increase rendering speed, they require significantly more memory than implicit volumetric representations. Hierarchical structure representations using octrees offer a sparse encoding of the 3D scene but still exhibit high memory occupancy. Recent work has addressed training models with neural sparse voxel fields~\cite{liu2020neural}, progressively reducing voxel granularity and skipping rendering for empty voxels. However, these approaches primarily focus on performance enhancement and artifact reduction rather than compression.

% %%%%% Methodology section starts here

% % \begin{figure*}[t]
% % \includegraphics[width=\linewidth]{Figures/playroom-pruning-comp.pdf}
% %     \centering
% %     \caption{Qualitative comparison of the playroom scene at various pruning levels, defined by $\gamma$ using gradient-aware iterative pruning. Our proposed method demonstrates substantially higher compression rates compared to both baselines while maintaining similar visual quality.}
% %     \label{fig: Pruning-Comparison-2}
% %     %\vspace{-0.4cm}
% % \end{figure*}


% % \begin{figure*}[t]
% % \includegraphics[width=\linewidth]{Figures/train-pruning-comp.pdf}
% %     \centering
% %     \caption{Qualitative comparison of the train scene at various pruning levels, defined by $\gamma$ using gradient-aware iterative pruning. Our proposed method demonstrates substantially higher compression rates compared to both baselines while maintaining similar visual quality.}
% %     \label{fig: Pruning-Comparison-3}
% %     %\vspace{-0.4cm}
% % \end{figure*}
% \subsection{3DGS Compression}
% \label{sec:3dgs-compress}
% When compared to NeRFs, 3DGS models lack structure, which presents challenges for compression~\cite{chen2024hac,fei20243d}. Consequently, many studies in 3DGS compression introduce structural parameters by replacing vanilla 3DGS parameters to enhance compression~\cite{lu2023scaffold, chen2024hac}. Scaffold-GS~\cite{lu2023scaffold}, for instance, utilizes anchor points to distribute local 3D Gaussians and predicts their attributes dynamically based on the viewing direction and distance within the view frustum. On the other hand, the Hash-grid Assisted Context (HAC)~\cite{chen2024hac} framework jointly learns a structured compact hash grid and uses it for context modeling of anchor attributes. %Specifically, with Scaffold-GS~\cite{lu2023scaffold} as their base model, for each anchor, they query the hash grid by the anchor location to obtain an interpolated hash feature, which is then used to predict the value distributions of anchor attributes, facilitating entropy coding.

% Niedermayr~\etal~\cite{niedermayr2023compressed} proposed a compression framework that maintains vanilla 3DGS parameters while compressing directional colors and Gaussian parameters. This framework incorporates sensitivity-aware vector clustering and quantization-aware training and achieves compression rates of up to 30$\times$ with a marginal decline in performance compared to the baseline 3DGS. Another method, Compact3D~\cite{lee2023compact}, introduces a learnable mask strategy to prune the Gaussians and a compact representation of view-dependent colors by employing a grid-based neural field rather than relying on spherical harmonics. It also learns codebooks to compactly represent the geometric attributes of Gaussian by vector quantization.

% Our proposed pruning method can effectively improve/replace the masking strategies for unimportant Gaussians in the existing works (see Sec.~\ref{sec:res}). However, for the scope of this paper and considering the broad applicability of vanilla 3DGS, we focus solely on the vanilla 3DGS variant.

% % \salman{When compared to NeRFs, 3D Gaussian Splatting (3DGS) models lack structure, posing challenges for compression. Consequently, the majority of studies in 3DGS compression introduce structural parameters by replacing vanilla 3DGS parameters to enhance compression~\cite{lu2023scaffold, fan2023lightgaussian, lee2023compact, chen2024hac, morgenstern2023compact}. Niedermayr et al.~\cite{niedermayr2023compressed} proposed a compression framework that maintains vanilla 3DGS parameters while compressing directional colors and Gaussian parameters. This framework incorporates sensitivity-aware vector clustering and quantization-aware training and achieves compression rates of up to 30$\times$ with a marginal decline in performance compared to the baseline 3DGS. Our pruning approach can seamlessly integrate with these end-to-end compression methods. However, for the scope of this paper and considering the broad applicability of vanilla 3DGS, we focus solely on the vanilla 3DGS variant.}

% \section{Methodology}
% %Despite the impressive performance and enhanced editability of 3DGS models, their substantial storage memory requirements often pose challenges, necessitating significant memory resources. 
% In this section, we first provide an overview of the 3DGS technique for learning and rendering 3D scenes, as introduced by Kerbl~\etal~\cite{kerbl20233d} (Sec.~\ref{sec: 3DGS}). Then, we delve into an explanation of our pruning approach (Sec.~\ref{sec: pruning}). Our methodology, depicted in Fig.~\ref{fig:overview}, introduces an effective approach to compress these models using gradient-informed pruning.
% %In this section, we first provide an overview of the 3D Gaussian Splatting (3DGS) technique for learning and rendering 3D scenes, as introduced by Kerbl et al.~\cite{kerbl20233d} (Sec~\ref{sec: 3DGS}). Despite their remarkable performance and enhanced editability, 3DGS models are hindered by their considerable storage memory requirements, often necessitating substantial memory resources. Our methodology, outlined in Figure \ref{fig:overview}, introduces a simple yet effective approach to compress these models using pruning technique (Sec~\ref{sec: pruning}).
% %First, we present an overview of the 3D Gaussian Splatting (3DGS)~\cite{kerbl20233d} technique for learning and rendering 3D scenes, followed by an explanation of our pruning approach.


% \subsection{Differentiable Gaussian Splatting}
% \label{sec: 3DGS}
% 3DGS~\cite{kerbl20233d} represents a scene through a set of 3D Gaussians. By leveraging differentiable Gaussian splatting, which extends EWA volume splatting~\cite{zwicker2001ewa}, it facilitates the efficient projection of 3D Gaussian kernels onto the 2D image plane. Additionally, differentiable rendering optimizes the quantity and attributes of the Gaussian kernels employed to characterize the scene. Each 3D Gaussian is characterized by its position and covariance matrices within the 3D space, modeled as
% %\vspace{-10pt}
% \begin{equation}
% G(x)=\exp\left[-\frac{1}{2}(x-\mu)^T \Sigma^{-1}(x-\mu)\right],
% %\vspace{-5pt}
% \end{equation}

% where \(x\) denotes the position vector, \(\mu\) represents the position, and \(\Sigma\) is the 3D covariance matrix of the Gaussian distribution. Given the requirement for the covariance matrix to be positive definite, it can be parameterized using a rotation matrix \(R\) and a scaling matrix \(S\). To facilitate independent optimization of \(R\) and \(S\), Kerbl~\etal~\cite{kerbl20233d} introduce a representation of rotation via a quaternion \(q\) and scaling through a vector \(s\), both of which can be converted into their corresponding matrices. Additionally, each Gaussian distribution possesses its opacity (\(\alpha \in [0, 1]\)) and a set of spherical harmonics (SH) coefficients essential for reconstructing a view-dependent color. The 2D projection of a 3D Gaussian remains a Gaussian with covariance
% \begin{equation}
%     \Sigma' = JW\Sigma W^TJ^T,
%     %\vspace{-5pt}
% \end{equation}
% \noindent
% where \(W\) is the view transformation matrix, and \(J\) is the Jacobian of the affine approximation of the projective transformation. This setup facilitates the evaluation of the 2D color and opacity footprint of each projected Gaussian. The color \(C\) of a pixel is subsequently determined by blending all the \(N\) 2D Gaussians contributing to that pixel:%, %with blending performed in sorted order thanks to the GPU efficient rasterization process, 
% %defined as
% %\vspace{-10pt}
% \begin{equation}
%     C = \sum_{i \in N} c_i \alpha_i + \prod_{j=1}^{i-1} (1 - \alpha_j),
% \end{equation}

% \noindent
% where \(c_i\) and \(\alpha_i\) represent the view-dependent color and opacity of a Gaussian, respectively, which are adjusted based on the exponential decay from the center point of the projected Gaussian. The parameters such as position \(x\), rotation \(q\), scaling \(s\), opacity \(\alpha\), and spherical harmonics (SH) coefficients of each 3D Gaussian are optimized to ensure alignment between the rendered 2D Gaussians and the training images.

% During the training phase, the 3D Gaussian splats are rendered efficiently in a differentiable manner to produce a 2D image. This rendering process involves $\alpha$-blending of anisotropic splats, sorting them, and utilizing a tile-based rasterizer. At each training iteration, the 3DGS framework renders the training viewpoints and then minimizes the loss between the ground truth and rendered images in the pixel space, where the loss is given by 
% %\vspace{-5pt}
% \begin{equation}
% \mathcal{L}=(1-\lambda) \mathcal{L}_1+\lambda \mathcal{L}_{\text {D-SSIM }},
% %\vspace{-5pt}
% \end{equation}

% \noindent
% %$\lambda$= 0.2 is employed consistently across all our experiments. For more details please refer to the 3DGS paper \cite{kerbl20233d}.
% where $\mathcal{L}_1$ is the $\ell_1$ norm of the rendered output and $\mathcal{L}_{\text {D-SSIM }}$ is its structural dissimilarity. The optimization in 3DGS begins with a point cloud generated through a conventional SfM method~\cite{ullman1979interpretation}, and then proceeds iteratively, pruning Gaussians with small opacity parameters and introducing new ones when significant gradients are detected. As demonstrated in the 3DGS paper, this approach enables rapid training and facilitates real-time rendering, all while achieving comparable or superior 3D model quality compared to state-of-the-art NeRF methods.

% %\subsection{Compressing Gaussian Splats}
% %While 3DGS models exhibit impressive performance and offer enhanced editability, they suffer from significant storage memory requirements, often demanding substantial memory resources. In our methodology as shown in \cref{fig:overview}, we introduce a straightforward yet powerful approach to compress these models using pruning technique.


% % \begin{table*}[t]

% %     \centering
% %     \scalebox{0.99}{
% %     \begin{tabular}{cccc|cccc}
% %     \toprule
% %     \multicolumn{4}{c}{One Shot Pruning} & \multicolumn{4}{c}{Iterative Pruning} \\
% %     SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem  &SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem \\
% %     \midrule
% %     0.848 & 23.920 & 0.171 & 326.75 & 0.849 & 23.981 & 0.169 & 338.5 \\
% %     0.848 & 23.901 & 0.172 & 261.5 & 0.849 & 23.939 & 0.171 & 261 \\
% %     0.844 & 23.813 & 0.180 & 196.25 & 0.846 & 23.961 & 0.178 & 200 \\
% %     0.839 & 23.698 & 0.191 & 152.75 & 0.839 & 23.799 & 0.192 & 152 \\
% %     0.819 & 23.376 & 0.228 & 87.5 & 0.818 & 23.404 & 0.232 & 86 \\
% %     0.793 & 22.927 & 0.272 & 44 & 0.794 & 23.069 & 0.574 & 47 \\
% %     0.756 & 22.234 & 0.322 & 22 & 0.767 & 22.655 & 0.310 & 25 \\
% %     \bottomrule
% %     \end{tabular}    
% %     }
% %     \caption{Performance comparison between one-shot pruning and iterative pruning on Tanks\&Temples dataset. Memory size is in MBs.}
% %     \label{tab: one-shot-pruning_comp}
% % \end{table*}

% % \begin{table}[t]
% %     \centering
% %     \scalebox{0.75}{
% %     \begin{tabular}{cccc|cccc}
% %     \toprule
% %     \multicolumn{4}{c}{One Shot Pruning} & \multicolumn{4}{c}{Iterative Pruning} \\
% %     SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem  &SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem \\
% %     \midrule
% %     0.848 & 23.920 & 0.171 & 326.75 & 0.849 & 23.981 & 0.169 & 338.50 \\
% %     0.848 & 23.901 & 0.172 & 261.50 & 0.849 & 23.939 & 0.171 & 261.00 \\
% %     0.844 & 23.813 & 0.180 & 196.25 & 0.846 & 23.961 & 0.178 & 200.00 \\
% %     0.839 & 23.698 & 0.191 & 152.75 & 0.839 & 23.799 & 0.192 & 152.00 \\
% %     0.819 & 23.376 & 0.228 & 87.50 & 0.818 & 23.404 & 0.232 & 86.00 \\
% %     0.793 & 22.927 & 0.272 & 44.00 & 0.794 & 23.069 & 0.574 & 47.00 \\
% %     0.756 & 22.234 & 0.322 & 22.00 & 0.767 & 22.655 & 0.310 & 25.00 \\
% %     \bottomrule
% %     \end{tabular}    
% %     }
% %     \caption{Performance comparison between one-shot pruning and iterative pruning on Tanks\&Temples dataset. Memory size is in MBs.}
% %     \label{tab:one-shot-pruning_comp}
% % \end{table}

% % \begin{table*}


% %     \centering
% %     \scalebox{0.99}{
% %     \begin{tabular}{cccc|cccc}
% %     \toprule
% %     \multicolumn{4}{c}{Opacity Aware Pruning} & \multicolumn{4}{c}{Gradient Aware Opacity Pruning} \\
% %     SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem  &SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & Mem \\
% %     \midrule
% %         0.849 & 23.981 & 0.169 & 338.5 & 0.849 & 23.962 & 0.170 & 335.5 \\
% %         0.849 & 23.939 & 0.171 & 261 & 0.849 & 23.971 & 0.171 & 280.75 \\
% %         0.846 & 23.961 & 0.178 & 200 & 0.848 & 23.966 & 0.175 & 219.25 \\
% %         0.839 & 23.799 & 0.192 & 152 & 0.844 & 23.936 & 0.187 & 153 \\
% %         0.818 & 23.404 & 0.232 & 86 & 0.829 & 23.848 & 0.220 & 76.75 \\
% %         0.794 & 23.069 & 0.574 & 47 & 0.810 & 23.559 & 0.251 & 45.25 \\
% %         0.767 & 22.655 & 0.310 & 25 & 0.780 & 22.919 & 0.294 & 23.375 \\
% %         0.731 & 21.902 & 0.354 & 12.65 & 0.761 & 22.511 & 0.319 & 14.75 \\
% %     \bottomrule
% %     \end{tabular}
% %     }
% %     \caption{Performance comparison between opacity aware pruning and gradient aware opacity pruning on Tanks\&Temples dataset. Memory size is in MBs.}
% %     \label{tab: gradient aware pruning}
% % \end{table*}



% \subsection{Gradient Aware Pruning}
% \label{sec: pruning}
% 3DGS typically necessitates several million Gaussians to adequately model a standard scene, each Gaussian entailing 59 parameters. This results in a storage size significantly larger than that of most NeRF methodologies, such as Mip-NeRF360~\cite{barron2022mip}, K-planes~\cite{fridovich2023k}, and InstantNGP~\cite{muller2022instant}. Such requirements render 3DGS inefficient for certain applications, particularly those involving edge devices. Our primary focus is on parameter reduction. In the original training process of 3DGS, Kerbl~\etal~\cite{kerbl20233d} pruned and densified Gaussians up to a specified number of iterations, with pruning based on a predetermined opacity threshold. However, if their opacity is low and so is its gradient, we can say they can be removed with little to no impact on the quality of the rendered scene. As such, we have 

% % \begin{equation}
% %     \label{eq: pruning}
% %     \boldsymbol{\Sigma}' = \begin{cases}\Sigma_i & \text { if } \left( \left|\Sigma_i\right|>\mathcal{Q}_{|\boldsymbol{\alpha}|}(\gamma)\right) \lor \left( \left|\Sigma_i\right| > \mathcal{Q}_{|\boldsymbol{\nabla\mathcal{L}}|}(\gamma) \right)
% %     \\ 0 & \text { otherwise, }\end{cases}
% % \end{equation}

% % \begin{equation}
% %     \label{eq: pruning}
% %     \boldsymbol{\Sigma}' = \begin{cases}\Sigma_i & \text { if } \left( \left|\Sigma_i\right|\geq \mathcal{Q}_{|\boldsymbol{\alpha}|}(\gamma)\right) \lor \left( \left|\Sigma_i\right| \geq \mathcal{Q}_{|\boldsymbol{\nabla\mathcal{L}}|}(\gamma) \right)
% %     \\ 0 & \text { if } \left( \left|\Sigma_i\right|<\mathcal{Q}_{|\boldsymbol{\alpha}|}(\gamma)\right) \land \left( \left|\Sigma_i\right| < \mathcal{Q}_{|\boldsymbol{\nabla\mathcal{L}}|}(\gamma) \right),
    
% %     \end{cases}
% % \end{equation}


% % \begin{equation}
% %     \label{eq: pruning}
% %     \boldsymbol{\Sigma}' = \begin{cases}\Sigma_i & \text { if } \left( \left|\Sigma_{i}\left(\alpha \right)\right|\geq \mathcal{Q}_{|\boldsymbol{\Sigma_{i}\left(\alpha \right)}|}(\gamma)\right) \lor \left( \left|\nabla\Sigma_i\right| \geq \mathcal{Q}_{|\boldsymbol{\nabla\Sigma^i}|}(\gamma) \right)
% %     \\ 0  & \text { otherwise, }
    
% %     \end{cases}
% % \end{equation}
% %\vspace{-5pt}
% \begin{equation}
%     \label{eq: pruning}
%     \boldsymbol{\Sigma}' = \begin{cases}
%      \Sigma_i & \text{if } \left[\left|\Sigma_i^\alpha\right|\geq \mathcal{Q}_{|\boldsymbol{\Sigma^\alpha}|}(\gamma_{\text{iter}})\right] \lor    \left[ \left|\nabla\Sigma_i\right| \geq \mathcal{Q}_{|\boldsymbol{\nabla\Sigma}|}(\gamma_{\text{iter}}) \right] \\
%     0  & \text{otherwise,}
%     \end{cases}
% \end{equation}



% \noindent where $\Sigma_i^\alpha$ denotes the $\alpha$ value of the $i$-th Gaussian, and $\nabla\Sigma_i$ denotes the gradient for the $i$-th Gaussian, $\mathcal{Q}_{|\boldsymbol{\Sigma^\alpha}|}(.)$ represents the quantile function for the opacity, $\mathcal{Q}_{|\boldsymbol{\nabla\Sigma}|}(.)$ is the quantile function for the gradients of the Gaussians, and $\gamma \in [0, 1]$ denotes the fraction of Gaussians to be removed. 
% %Through \eqref{eq: pruning}, we generate masks based on opacity and gradient separately and subsequently apply pruning solely on those Gaussians for which both masks evaluate to True. At a glance, to prune a specific Gaussian, it is necessary for both its opacity and gradient values to fall below the quantile threshold defined by $\gamma$. 
% This pruning process, along with periodic fine-tuning, not only improves performance but evidently results in substantial compression gains.

% %where $\mathcal{Q}_{|\boldsymbol{\alpha}|}(\cdot)$ represents the quantile function for the opacity of the Gaussians, while $\mathcal{Q}_{|\boldsymbol{\nabla\mathcal{L}}|}(.)$ signifies the quantile function for the gradients. $\gamma \in [0, 1]$ denotes the fraction of Gaussians to be removed. Utilizing the above \cref{eq: pruning}, we generate masks based on opacity and gradient separately and subsequently apply pruning solely on those Gaussians for which both masks evaluate to True. Put simply, to prune a specific Gaussian, it is necessary for both its opacity and gradient values to fall below the quantile threshold defined by $\gamma$. This pruning process, along with periodic fine-tuning, not only improves performance but also results in substantial compression gains.

% %where $\mathcal{Q}_{|\boldsymbol{\alpha}|}(\cdot)$ denotes the quantile function for the opacity of the Gaussians, with $\gamma \in [0, 1]$ representing the fraction of Gaussians to be removed. This pruning process, along with periodic fine-tuning, not only improves performance but also results in substantial compression gains.

% The iterative pruning and fine-tuning approaches enable the removal of redundant Gaussians while refining the remaining ones to better capture scene details compared to the baseline. Prior research in scene rendering has demonstrated that a gradual iterative pruning strategy can yield significantly sparser models while preserving high fidelity~\cite{deng2023compressing}. However, the impact of such an approach on 3DGS models yet remains unclear. We speculate that by gradually pruning the model over a specified number of iterations $t$ and aiming for a target sparsity $\gamma_{\text{target}}$, we can achieve improved results through a sparsification process applied to the 3DGS model: at every iteration, we apply the sparsification
% \begin{equation}
%     \gamma_{\text{iter}} = 1 - (1-\gamma_{\text{target}})^{\frac{1}{t}}.
% \end{equation}
% \noindent Our approach is based on two key factors. First, during the fine-tuning stage following pruning, the covariance $\Sigma$ is adjusted to minimize rendering loss, leading to higher values for solid surfaces and lower values for semi-transparent artifacts, which can be subsequently removed in the next iteration (which will be empirically observed in Fig.~\ref{fig: iterative vs one-shot}c). Second, the gradual iterative process helps prevent the optimization algorithm from converging to sub-optimal local minima (according to empirical evidence discussed in Sec.~\ref{sec:abl}). Hence, it is crucial to initiate the process with an overparametrized yet well-performing model. Similar observations can be drawn from traditional deep learning literature~\cite{blalock2020state, woodworth2020kernel}. In the next section, we will present a quantitative analysis of typical benchmarks employed for 3DGS.

% %%%% Results section starts here
% % \begin{figure}
% % \includegraphics[width=0.85\linewidth]{Figures/Gradient Aware.pdf}
% %     \centering
% %     \caption{The graph illustrates the performance-size trade-off obtained through opacity-aware pruning and gradient-aware opacity pruning on the Tanks\&Temple dataset. Both methods demonstrate considerable enhancements in performance and compression compared to the 3DGS-30k and 3DGS-7k baselines. Notably, gradient-aware pruning exhibits substantial performance improvement at lower compression rates.}
% %     \label{fig: gradient aware}
% %     \vspace{-0.4cm}
% % \end{figure}

% % \begin{table*}[ht]
% %     \caption{Performance comparison using gradient-aware iterative pruning with different pruning levels defined by $\gamma$ against 3DGS-30k, 3DGS-7k baselines, and opacity-based iterative pruning. $^*$Reproduced using official code. $^\dag$ Reported from~\cite{kerbl20233d}. Memory size is in MBs.
% %     %Comparison of performance using opacity-aware iterative pruning with different pruning levels defined by $\gamma$ against 3DGS-30k and 3DGS-7k baselines. $^*$Reproduced using official code. $^\dag$ Reported from \cite{kerbl20233d}. Memory size is in MBs.
% %     %Comparison of performance using opacity-aware iterative pruning with different pruning levels defined by $\gamma$ against 3DGS-30k and 3DGS-7k baselines. $^*$Reproduced using official code. $^\dag$ Reported from \cite{kerbl20233d}. Memory size is in MBs
% %     }
% %     \label{tab:pruning_comp}
% %     \centering
% %     \resizebox{\textwidth}{!}{
% %     \begin{tabular}{l|c|cccc|cccc|cccc}
% %     \toprule
% %       &   & \multicolumn{4}{c}{Mip-NeRF360} & \multicolumn{4}{c}{Tanks\&Temples} & \multicolumn{4}{c}{Deep Blending} \\
% %     \textbf{Model} & \textbf{$\boldsymbol{\gamma}$} & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\downarrow$ & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\downarrow$ & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\downarrow$ \\
% %     \midrule
    
% %    3DGS-7k$^\dag$ & -   & 0.770 & 25.60 & 0.279 & 523.00 &0.767 & 21.20 & 0.280 & 270.00 & 0.875 & 27.78 & 0.317 & 386.00 \\
% %     3DGS-30k$^\dag$ & -     & 0.815 & 27.21 & 0.214 &    734.00   & 0.841 & 23.14 & 0.183 &  411.00  & 0.903 & 29.41 & 0.243 & 676.00 \\
% %     3DGS-7k$^*$   & -    & 0.765 & 25.88 & 0.288 & 541.70  & 0.777 & 21.66 & 0.266 & 298.00 &  0.876 & 28.26 & 0.312 & 410.50  \\
% %     3DGS-30k$^*$ & -     & 0.812 & 27.46 & 0.221 & 763.40  & 0.845 & 23.69 & 0.178 & 435.50 & 0.899 & 29.51 & 0.246 & 664.50 \\
% % \midrule
% %     \multirow{8}{*}{\begin{tabular}{@{}p{2cm}@{}}3DGS-Opacity Based \\ Pruning\end{tabular}} & 0.025 & 0.813 & 27.58 & 0.217 & 592.22 & 0.849 & 23.98 & 0.169 & 338.50 & 0.894 & 29.27 & 0.248 & 516.00 \\
% %     & 0.050 & 0.813 & 27.56 & 0.220 & 449.11 & 0.849 & 23.94 & 0.171 & 261.00 & 0.894 & 29.27 & 0.250 & 398.00 \\
% %     & 0.075 & 0.809 & 27.47 & 0.231 & 344.00 & 0.846 & 23.96 & 0.178 & 200.00 & 0.895 & 29.27 & 0.252 & 305.00 \\
% %     & 0.100 & 0.799 & 27.25 & 0.250 & 261.78 & 0.839 & 23.80 & 0.192 & 152.00 & 0.894 & 29.22 & 0.259 & 232.00 \\
% %     & 0.150 & 0.762 & 26.46 & 0.304 & 148.00 & 0.818 & 23.40 & 0.232 & 86.00 & 0.888 & 28.96 & 0.279 & 131.00 \\
% %     & 0.200 & 0.725 & 25.66 & 0.353 & 80.89 & 0.794 & 23.07 & 0.574 & 47.00 & 0.883 & 28.66 & 0.295 & 72.00 \\
% %     & 0.250 & 0.692 & 24.98 & 0.394 & 42.78 & 0.767 & 22.66 & 0.310 & 25.00 & 0.877 & 28.20 & 0.310 & 38.00 \\
% %     & 0.300 & 0.659 & 24.26 & 0.430 & 22.14 & 0.731 & 21.90 & 0.354 & 12.65 & 0.869 & 27.69 & 0.328 & 19.00 \\
% % \midrule
% %     \multirow{8}{*}{\begin{tabular}{@{}p{2cm}@{}}3DGS-Gradient Aware \\ Pruning\end{tabular}} & 
% %     0.225 & 0.813 & 27.60 & 0.217 & 543.44 & 0.849 & 23.96 & 0.170 & 335.50 & 0.894 & 29.28 & 0.248 & 534.00 \\
% % & 0.275 & 0.814 & 27.60 & 0.219 & 464.33 & 0.849 & 23.97 & 0.171 & 280.75 & 0.894 & 29.26 & 0.248 & 481.50 \\
% % & 0.325 & 0.813 & 27.60 & 0.223 & 386.11 & 0.848 & 23.97 & 0.175 & 219.25 & 0.895 & 29.29 & 0.249 & 416.00 \\
% % & 0.375 & 0.810 & 27.56 & 0.231 & 311.78 & 0.844 & 23.94 & 0.187 & 153.00 & 0.895 & 29.29 & 0.250 & 339.00 \\
% % & 0.450 & 0.797 & 27.33 & 0.256 & 194.22 & 0.829 & 23.85 & 0.220 & 76.75 & 0.897 & 29.34 & 0.253 & 205.50 \\
% % & 0.500 & 0.776 & 26.92 & 0.288 & 119.44 & 0.810 & 23.56 & 0.251 & 45.25 & 0.898 & 29.37 & 0.258 & 118.50 \\
% % & 0.550 & 0.740 & 26.15 & 0.336 & 63.56 & 0.780 & 22.92 & 0.294 & 23.38 & 0.896 & 29.16 & 0.269 & 59.00 \\
% % & 0.600 & 0.690 & 25.03 & 0.394 & 29.22 & 0.761 & 22.51 & 0.319 & 14.75 & 0.887 & 28.62 & 0.293 & 25.50 \\
% %     \bottomrule


    
% %     \end{tabular}
% %     }
% % \end{table*}


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{Figures/Gradient Aware Comparison_updated.pdf}
%     %\vspace{-10pt}
%     \caption{The graph depicts the trade-off between performance and size when utilizing Trimming the Fat (gradient-aware iterative pruning) compared to the 3DGS-30k and 3DGS-7k baselines as well as opacity-based pruning on the Mip-NeRF360, Tanks\&Temple, and Deep Blending datasets.}
%     \label{fig: comparison}
% \end{figure*}

% % \begin{wrapfigure}{r}{0.5\textwidth}
% % \centering
% % \vspace{-0.4cm}
% % \includegraphics[width=0.9\linewidth]{Figures/FPS Comparison.pdf}
    
% %     \caption{\salman{The graph illustrates the performance-size trade-off achieved by our method compared to the pruning approach proposed in Compact 3D~\cite{lee2023compact} on the Tanks\&Temple and Mip-NeRF360 datasets.}}
% %     \label{fig: FPS}
% %     \vspace{-0.4cm}
% % \end{wrapfigure}

% % \begin{wrapfigure}{r}{0.5\textwidth}
% % \centering
% % \vspace{-0.4cm}
% % \includegraphics[width=0.9\linewidth]{Figures/Pruning vs 3DCompact.pdf}
    
% %     \caption{\salman{The graph illustrates the performance-size trade-off achieved by our method compared to the pruning approach proposed in Compact 3D~\cite{lee2023compact} on the Tanks\&Temple and Mip-NeRF360 datasets.}}
% %     \label{fig: pruning vs 3DCompact}
% %     \vspace{-0.4cm}
% % \end{wrapfigure}

% % \begin{figure}[!htb]
% %     \centering
% %     \begin{minipage}[t]{0.22\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{Figures/Tanks and Temple FPS.pdf}
% %         \caption{\salman{The graph illustrates the effectiveness of our proposed method in enhancing the FPS of 3DGS.}}
% %         \label{fig: FPS}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.22\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{Figures/Tanks and Temple vs Compact3D.pdf}
% %         \caption{\salman{The graph illustrates the performance-size trade-off achieved by our method compared to the pruning approach proposed in Compact 3D~\cite{lee2023compact} on the Tanks\&Temple and Mip-NeRF360 datasets.}}
% %         \label{fig: pruning vs 3DCompact}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.22\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{Figures/Tanks and Temple vs Compact3D.pdf}
% %         \caption{\salman{The graph illustrates the performance-size trade-off achieved by our method compared to the pruning approach proposed in Compact 3D~\cite{lee2023compact} on the Tanks\&Temple and Mip-NeRF360 datasets.}}
% %         \label{fig: pruning vs 3DCompact}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.22\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{Figures/Tanks and Temple vs Compact3D.pdf}
% %         \caption{\salman{The graph illustrates the performance-size trade-off achieved by our method compared to the pruning approach proposed in Compact 3D~\cite{lee2023compact} on the Tanks\&Temple and Mip-NeRF360 datasets.}}
% %         \label{fig: pruning vs 3DCompact}
% %     \end{minipage}
% % \end{figure}


% \begin{figure*}[t]
% \includegraphics[width=0.85\linewidth]{Figures/mip-nerf-visual.pdf}
%     \centering
%     %\vspace{-5pt}
%     \caption{Qualitative comparison of the garden scene at various pruning levels ($\gamma$) using gradient-aware iterative pruning. Our proposed method demonstrates substantially higher compression rates compared to both baselines while maintaining similar visual quality.}
%     \label{fig: Pruning-Comparison-1}
%     %\vspace{-0.4cm}
% \end{figure*}




% \section{Experiments and Results}
% %\vspace{-0.2cm}
% In this section, we present our empirical findings on commonly recognized benchmarks within the 3DGS community. We begin by detailing the implementation of our approach, followed by an outline of the benchmarked datasets and the evaluation metrics employed (Sec.~\ref{sec:idf}). Subsequently, we discuss both qualitative and quantitative results (Sec.~\ref{sec:res}), providing as well an ablation study (Sec.~\ref{sec:abl}).

% \subsection{Implementation Details}
% \label{sec:idf}
% %In all our experiments, we utilize the publicly available official code repository of 3DGS \cite{kerbl20233d} without making any alterations to the hyperparameters used for training, ensuring consistency with the original 3DGS model.
% In all our experiments, we use the publicly available official code repository of 3DGS~\cite{kerbl20233d}, adhering to the recommended hyperparameter settings used for training to maintain consistency with the original 3DGS model. We initiate the pruning process with the optimized Gaussians trained for 30,000 iterations, employing pruning with %$\gamma = [0.225, 0.275, 0.325, 0.375, 0.45, 0.5, 0.55, 0.6]$
% $\gamma_{\text{iter}}\in[0.225,0.6]$, as described in \eqref{eq: pruning}.  Iterative pruning with the same $\gamma_{\text{iter}}$ value is applied after every 500 iterations until reaching 35,000 iterations (commencing from 30,000 iterations), followed by further fine-tuning for 10,000 iterations. For all our experiments, pruning and fine-tuning consistently yield significantly improved compression-performance trade-offs. Additionally, $\lambda= 0.2$ is employed consistently across all our experiments. 

% %For all our experiments, we employ the publicly available official code repository of 3D Gaussian Splat \cite{kerbl20233d}, without modifying the hyperparameters used for training compared to the original 3D Gaussian Splat model. We begin the pruning process with the optimized Gaussians trained for 30,000 iterations, applying pruning using \eqref{eq: pruning} with $\gamma$, where $~{\gamma = [0.225, 0.275,0.325,0.375,0.45,0.5,0.55,0.6]}$. The model undergoes sequential pruning with the same $\gamma$ value after every 1000 iterations until reaching 40,000 iterations (starting from 30,000 iterations), followed by further finetuning for 20,000 iterations. In most experiments, pruning and finetuning result in superior performance compared to the baseline.
% \noindent\textbf{Datasets.} We assess the efficacy of our pruning approach across diverse scenes, encompassing environments from the Mip-Nerf360~\cite{barron2022mip} indoor and outdoor datasets, alongside two scenes sourced from the Tanks\&Temples~\cite{knapitsch2017tanks} and Deep Blending~\cite{hedman2018deep} datasets, akin to the scenes examined in the original 3DGS work~\cite{kerbl20233d}.

% \noindent\textbf{Evaluation.} To ensure a fair comparison, we adhere to the same train-test split utilized in Mip-Nerf360~\cite{barron2022mip} and 3DGS~\cite{kerbl20233d}. %Moreover, we include our reproduced metrics for 3DGS, as we observed slightly enhanced results compared to those reported in~\cite{kerbl20233d} for certain scenes when executing their code ourselves. 
% Our evaluation encompasses standard metrics like SSIM, PSNR, and LPIPS, alongside the average memory consumption across all datasets.


% \subsection{Results}
% \label{sec:res}
% \subsubsection{Quantitative Comparison} 
% \textbf{Trimming the Fat.} We conduct a comparative analysis between our method, the 3DGS-30k, and 3DGS-7k baselines, along with an opacity-based pruning approach that removes gradient information from \eqref{eq: pruning}. As illustrated in Fig.~\ref{fig: comparison}, we examine the trade-off in compression performance across benchmark datasets. Across all the datasets, Gaussian splats can be pruned by up to 4$\times$, showcasing improved or similar performance compared to the baseline. Notably, even at significantly high pruning levels, where the average scene size is less than 25MB, our proposed pruning technique maintains comparable or even superior performance to that of the 3DGS-7k variant, achieving compression rates of up to 24$\times$ on average. This is realized without the need for any additional end-to-end compression pipeline integration, highlighting the standalone scalability of our proposed approach. 
% %We compare our method with the 3DGS-30k and 3DGS-7k baselines, as well as with an opacity-based pruning approach, in which the gradient information from \cref{eq: pruning} is removed. Figure~\ref{fig: comparison} illustrate the tradeoff in compression performance across benchmark datasets. For the Tanks\&Temples and Mip-NeRF360 datasets, Gaussian splats can be pruned by up to 4$\times$ with improved or similar performance compared to the baseline. However, in the Deep Blending dataset, our best pruning model results in a negligible loss of about 0.07 PSNR. It is worth noting that a PSNR difference of 0.5 is imperceptible to the human eye \cite{salomon2010handbook}. Similarly, for Deep Blending, Gaussian splats can be pruned by more than 4$\times$ without a drop in performance. Further compression reveals information loss, yet our method maintains performance better/ similar to the 3DGS-7k baseline, achieving compression rates of up to 24$\times$ on average.

% Opacity-based pruning exhibits similar performance to gradient-aware pruning at small pruning thresholds. However, the performance difference becomes more pronounced at higher compression rates, as evident from the results in Fig.~\ref{fig: comparison}. Incorporating gradient information leads to additional performance improvements in pruning. This enhancement arises because certain scene features (sky, glass, etc.) may have low opacity but are still crucial for overall scene rendering. By considering gradient information, we ensure that only Gaussians containing unimportant features are pruned. Our proposal of incorporating information on the gradient shows its prominent effectiveness at higher pruning rates. For a more detailed comparison please refer to the supplementary material.

% \begin{figure}
%     \begin{tabular}{@{}c@{}c@{}c@{}}
%         \bmvaHangBox{\includegraphics[width=0.3\columnwidth]{Figures/One Shot Pruning vs Iterative Pruning (1).pdf}}&
%         \bmvaHangBox{\includegraphics[width=0.3\columnwidth]{Figures/Tanks and Temple FPS.pdf}}&
%         \bmvaHangBox{\includegraphics[width=0.4\columnwidth]{Figures/b_p_opacity (1).pdf}}\\
%         (a)&(b)&(c)\\
%     \end{tabular}
%     %\vspace{-10pt}
%     \caption{Trade-off between performance and size through iterative pruning and one-shot pruning techniques (a) and in terms of FPS on the Tanks\&Temples dataset (b), and opacity distribution before and after pruning for the \texttt{truck} scene (c).}% Both approaches exhibit significant improvements in performance and compression compared to the 3DGS-30k and 3DGS-7k baselines.}
%     \label{fig: iterative vs one-shot}
% \end{figure}
% %\begin{wrapfigure}{r}{0.4\textwidth}
% %\centering
% %\vspace{-0.4cm}

% %    
% %\end{wrapfigure}
% \noindent
% \textbf{Trimming the Fat with end-to-end compression.}
% Our proposed pruning methodology can act as a plug-and-play with various end-to-end compression techniques for 3DGS. When integrated with the method proposed by Niedermayr~\emph{et~al.}~\cite{niedermayr2023compressed}, we achieve state-of-the-art compression performance. Niedermayr's approach begins with a pre-trained Gaussian as the foundation of its compression process. We substitute this pre-trained Gaussian with our pruned Gaussian and apply the end-to-end compression procedure. This combination results in 50$\times$ compression compared to the baseline, while maintaining comparable performance. Moreover, we achieve 2$\times$ compression with improved performance compared to Niedermayr's original approach, as demonstrated in Table~\ref{tab:compression_comp}. %For initialization of our compression pipeline, we employ pre-trained scenes pruned at specific thresholds: $\gamma = 0.325$ for the Mip-NeRF360 dataset, $\gamma = 0.425$ for Tanks\&Temple, and $\gamma = 0.475$ for Deep Blending.

% %Table \ref{tab:pruning_comp} compares our method with the 3DGS-30k and 3DGS-7k baselines, while the \cref{fig: comparison} illustrates the tradeoff in compression performance across benchmark datasets. In the Tanks\&Temples and Mip-NeRF360 datasets, Gaussian splats can be pruned by up to half with better performance than the baseline. However, for the Deep Blending dataset, pruning results in an indiscernible loss of about 0.25 PSNR. It is important to note that a PSNR difference of 0.5 is indistinguishable to the human eye \cite{salomon2010handbook}. Similarly, for Deep Blending, Gaussian splats can be pruned by more than 50\% without a drop in performance. Information loss becomes evident with further compression. Nevertheless, even with very high compression rates, our method maintains performance similar to the 3DGS-7k baseline, achieving compression rates of up to 24$\times$ on average.
% %\vspace{-0.4cm}
% \subsubsection{Qualitative Comparison} We present visualizations of the \texttt{garden} scene from the Mip-NeRF360 dataset, which typically demands substantial memory resources. In Fig.~\ref{fig: Pruning-Comparison-1} we showcase the visualizations of test set images at various pruning levels denoted by $\gamma_{\text{iter}}$. Our gradient-aware iterative pruning pipeline demonstrates significant compression rates while maintaining comparable visual quality. Specifically, our method compresses the Gaussian splats by approximately $4\times$ with visual quality akin to 3DGS-30K. Moreover, with $\gamma_{\text{iter}}=0.60$, our method achieves a compression ratio of approximately 25$\times$ while preserving visual quality comparable to 3DGS-7K. For additional visualizations, please refer to the supplementary material.



% %We present visualizations of scenes from the Tanks \& Temples, Mip-NeRF360, and Deep Blending datasets, all of which require substantial memory resources on average. In \cref{fig: Pruning-Comparison-1,fig: Pruning-Comparison-2,fig: Pruning-Comparison-3}, we illustrate the visualizations of test set images at various pruning levels indicated by $\gamma$. Our gradient-aware iterative pruning pipeline achieves noteworthy compression rates while maintaining comparable visual quality. Across all scenes depicted in the \cref{fig: Pruning-Comparison-1,fig: Pruning-Comparison-2,fig: Pruning-Comparison-3}, our method compresses the Gaussian splats by approximately $4\times$ with visual quality similar to 3DGS-30K. Furthermore, with $\gamma=0.60$, our method achieves an average compression ratio of approximately 12$\times$ while preserving visual quality comparable to 3DGS-7K.

% \subsection{Ablation Study}
% \label{sec:abl}
% \textbf{FPS Gain with Trimming the Fat.} Our novel pruning approach significantly enhances the FPS rate of 3DGS. On the Tanks\&Temples dataset, our method achieves an FPS of over 600+ all while maintaining SOTA performance as shown in~Fig.~\ref{fig: iterative vs one-shot}b. The renderings were performed using an RTX-3090, and the final FPS reported were averaged over three separate runs. These findings demonstrate the scalability of our proposed method.% for low-powered edge devices.

% % \textbf{Trimming the Fat vs Compact3D~\cite{lee2023compact}.} \salman{Fig.~\ref{fig: iterative vs one-shot}b depicts a comparison of PSNR and Gaussian counts between our proposed approach and Compact 3D using the Tanks\&Temples dataset. The results unequivocally highlight the superior performance of our method, demonstrating its capability to significantly reduce the number of Gaussians while maintaining baseline performance levels. These findings emphasize the effectiveness of our pruning technique and its potential to advance or replace existing compression methodologies for 3DGS.} 

% %Figure~\ref{fig: pruning vs 3DCompact} illustrate the comparison of PSNR and the number of Gaussians between our approach and Compact 3D for the Tanks\&Temple dataset. The Fig.~\ref{fig: pruning vs 3DCompact} unequivocally demonstrate the superiority of our proposed method for the benchmark dataset. The results underscore the significance of our pruning approach compared to existing methods in the literature~\cite{lee2023compact}.}

% \noindent\textbf{Why 3D Prior for Pruning is important?}
% To assess the significance of a 3D prior in the pruning process, we modified the original training protocol introduced by Kerbl~\etal~\cite{kerbl20233d}. In their methodology, Gaussians are pruned and densified up to a specified iteration count (15k), employing an opacity threshold for pruning. Our modification involved halting the densification phase at the same iteration count (15k) but extending the pruning phase for an additional 10k iterations. Subsequently, the model underwent further fine-tuning for an additional 5k iterations to generate the final scene. The findings are outlined in Fig.~\ref{fig: iterative vs one-shot}a, indicating that even with a reduced pruning threshold, achieving convergence without a robust 3D prior remains challenging for a 3DGS model.%To assess the significance of a 3D prior in the pruning process, we adapted the original training protocol introduced by Kerbl et al.~\cite{kerbl20233d}. In their methodology, Kerbl et al. pruned and refined Gaussians up to a specified iteration count (15k), employing an opacity threshold for pruning. Our modification involved halting the refinement phase at the same iteration count (15k) but extending the pruning phase for an additional 10k iterations. Subsequently, the model underwent further fine-tuning for an additional 5000 iterations to generate the final scene. The findings are outlined in the~\cref{tab:3D-prior}, indicating that even with a reduced pruning threshold, achieving convergence without a robust 3D prior remains challenging for a 3DGS model.}

% \noindent\textbf{Why Pruning is effective?}
% Our proposed pruning technique achieves compression ratios of up to $4\times$ without compromising performance compared to the 3DGS baseline. The efficacy of our approach lies in its ability to effectively eliminate redundant Gaussians. As depicted in Fig.~\ref{fig: iterative vs one-shot}c, the opacity distribution before and after pruning for the \texttt{truck} changes significantly. For the baseline 3DGS, the majority of opacity values are very low, indicating minimal contribution to scene reconstruction. However, through post-hoc pruning, a significant proportion of opacity values become notably higher, indicating that a more solid geometry is learned by the model.

% \noindent\textbf{One Shot Pruning vs Iterative Pruning.}
% We also explored the impact of one-shot pruning in comparison to iterative pruning, in terms of model size, showcased in Fig.~\ref{fig: iterative vs one-shot}a. For one-shot pruning, we utilized the pre-trained 3DGS-30k model, performed the pruning process once, and then fine-tuned the model for 30k iterations. Both gradient-aware and opacity-based iterative pruning consistently outperformed the one-shot pruning method: our results demonstrate that gradual pruning enables the model to better adapt to the scene compared to one-shot pruning. %  The memory size reflects the effectiveness of pruning on the 3DGS, as depicted in Fig.~\ref{fig: iterative vs one-shot}a. 

% %We explored the impact of one-shot pruning in comparison to iterative pruning. Our results demonstrate that gradual pruning enables the model to better adapt to the scene compared to one-shot pruning. For one-shot pruning, we utilized the pretrained 3DGS-30k model, performed the pruning process once, and then fine-tuned the model for 30k iterations. Table \ref{tab:one-shot-pruning_comp} presents a comprehensive comparison between one-shot pruning and iterative pruning on the Tanks\&Temples dataset, while the compression performance tradeoff is visualized in \cref{fig: iterative vs one-shot}. The memory size reflects the effectiveness of pruning on the 3DGS, as depicted in both Table \ref{tab: one-shot-pruning_comp} and \cref{fig: iterative vs one-shot}.


% % \subsubsection{Lottery Ticket for the Gaussian Splats?}\enzo{this whole section lacks the experiment outcome!} We investigated the potential presence of a ``lottery ticket'' phenomenon~\cite{frankle2018lottery} for Gaussian splats. To test this hypothesis, we took an already pruned set of Gaussian splats from the Tanks\&Temples dataset and randomly reinitialized all learnable features, including spherical harmonics (SH) features, opacity, scale, and rotation. Subsequently, we attempted to train these Gaussian splats for 30,000 iterations, but they failed to converge. This experiment underscores the necessity of having a learned 3D prior to which redundant information can be pruned. It highlights the difficulty of training Gaussian splats with the minimum number of Gaussians without any prior information from the 3D scene.




% %\noindent\textbf{Gradient Aware Opacity Pruning:}
% %We also examined the influence of gradient information on opacity-aware pruning. In this analysis, we utilized the same threshold value, denoted by $\gamma$, for both calculating the mask based on gradient and opacity. The approach involved generating masks based on opacity and gradient separately and then pruning only those Gaussians for which both masks evaluated to true. In simpler terms, to prune a specific Gaussian, it was required that both its opacity and gradient values fell below the quantile threshold defined by $\gamma$. The results obtained from the Tanks\&Temples dataset are presented in both the Table~\ref{tab: gradient aware pruning} and \cref{fig: gradient aware}. The findings indicate that incorporating gradient information leads to further performance improvements in pruning. This enhancement stems from the fact that certain scene features may possess low opacity but are still crucial for overall scene rendering. By considering gradient information, we ensure that only Gaussians containing unimportant features are pruned. This effectiveness becomes more pronounced at higher pruning rates.

% %\vspace{-0.2cm}

% \begin{table}[t]
%     \caption{Performance and compression comparison of 3DGS baseline, end-to-end compression~\cite{niedermayr2023compressed}, and our proposed method with the reference end-to-end compression method. Comp. stands for compression rate. $^\dag$ Reported from~\cite{niedermayr2023compressed}. }
%     \label{tab:compression_comp}
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|ccccc|ccccc|ccccc}
%     \toprule
%       &  \multicolumn{5}{c}{3D Gaussian Splatting$^\dag$} & \multicolumn{5}{c}{End to End Compression~\cite{niedermayr2023compressed}$^\dag$} & \multicolumn{5}{c}{Our's Trimming the Fat with End to End Compression} \\
%     \textbf{Dataset} & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\downarrow$ & \textbf{Comp.}$^\uparrow$ & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} &  \textbf{Mem}$^\downarrow$ &  \textbf{Comp.}$^\uparrow$ & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\uparrow$ & \textbf{Comp.}$^\uparrow$\\
%     \midrule
    
%    Mip-NeRF360 & 0.812 & 27.287 & 0.220 & 795.263 & 1$\times$ &  0.801 & 26.981 & 0.238 & 28.803 & 26.230$\times$ & 0.798 & 27.130 & 0.248 & 20.057 & 39.650$\times$ \\
%    Tanks\&Temples & 0.838  & 23.355 & 0.186 & 421.906 &   1$\times$ &  0.832 & 23.343 & 0.194 & 17.282 &  23.260$\times$  & 0.831 & 23.689 & 0.210 & 8.555 & 49.317$\times$ \\
%    Deep Blending  & 0.898  & 29.432  & 0.246 & 703.772 & 1$\times$ & 0.898 & 29.381   & 0.253  & 25.299 & 27.816$\times$ &  0.897 & 29.425 & 0.267 & 12.494 & 56.329$\times$ \\

%     \bottomrule
%     \end{tabular}



    
%     }
% \end{table}


% % \begin{table}[t]
% %     \caption{\salman{Comparison between the baseline 3DGS-30k model, its variant with additional pruning, and the proposed method.}}
% %     \label{tab:3D-prior}
% %     \centering
% %     \resizebox{\textwidth}{!}{
% %     \begin{tabular}{l|cccc|cccc}
% %     \toprule
% %       &  \multicolumn{4}{c}{Train} & \multicolumn{4}{c}{Truck} \\
% %      Method & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} & \textbf{Mem}$^\downarrow$ & \textbf{SSIM$^\uparrow$} & \textbf{PSNR$^\uparrow$} & \textbf{LPIPS$^\downarrow$} &  \textbf{Mem}$^\downarrow$\\
% %     \midrule
% % 3DGS-30k Baseline & 0.710 & 19.481 & 0.331 & 257 & 0.878 & 25.313 & 0.147 & 614 \\
% % 3DGS-30k with Additional Pruning & 0.752 & 19.887 & 0.287 & 134 & 0.856 & 24.364 & 0.192 & 525 \\
% % Gradient Aware Pruning & 0.804 & 22.449 & 0.234 & 64 & 0.867 & 25.360 & 0.182 & 126 \\

% %     \bottomrule
% %     \end{tabular}
% %     }
% % \end{table}



% %  \begin{figure*}[t]
% %     \centering
% %     \includegraphics[width=1.0\linewidth]{Figures/Gradient Aware Comparison.pdf}
% %     \caption{The graph depicts the trade-off between performance and size when utilizing gradient-aware iterative pruning compared to the 3DGS-30k and 3DGS-7k baselines as well as opacity-based pruning on the Mip-NeRF360, Tanks\&Temple, and Deep Blending datasets.}
% %     \label{fig: comparison}
% % \end{figure*}

% %\vspace{-0.2cm}

% \section{Conclusion}
% In this work, we presented a gradient-aware iterative pruning technique for 3D Gaussian splats named after ``Trimming the fat''. Our method effectively scales down Gaussian splats by a factor 4$\times$ without sacrificing generative quality. Particularly at higher pruning levels, our proposed method achieves compression ratios of approximately 25$\times$ and achieves up to 600~FPS with minimal impact on generative performance across established benchmark datasets. The resulting highly compressed point clouds can be seamlessly transmitted over networks and utilized on resource-constrained devices, offering potential applications in mobile VR/AR and gaming. Future research directions include investigating the integration of quantization-aware training methods to further improve the compressibility of 3DGS.
% %We have presented an opacity-aware iterative pruning technique for 3D Gaussians. Our method effectively prunes Gaussian splats by half without sacrificing information, achieving compression ratios of approximately 25$\times$ with minimal impact on generative performance across established benchmark datasets. The significantly compressed Gaussian point cloud can be seamlessly streamed over networks and rendered on low-power devices, rendering it suitable for mobile VR/AR applications and games. Moving forward, we intend to explore the integration of gradient information to enhance the pruning pipeline further.

% \section*{Acknowledgements}
% This work was partially funded by Hi!PARIS Center on Data Analytics and Artificial Intelligence.

% \bibliography{main}
% \end{document}

